Cross-checking SMBH mass estimates in NGC 6958 -- I: Stellar dynamics from adaptive optics-assisted MUSE observations

Supermassive black hole masses (MBH) can dynamically be estimated with various methods and using different kinematic tracers. Different methods have only been cross-checked for a small number of galaxies and often show discrepancies. To understand these discrepancies, detailed cross-comparisons of additional galaxies are needed. We present the first part of our cross-comparison between stellar- and gas-based MBH estimates in the nearby fast-rotating early-type galaxy NGC 6958. The measurements presented here are based on ground-layer adaptive optics-assisted Multi-Unit Spectroscopic Explorer (MUSE) science verification data at around 0.6 arcsec spatial resolution. The spatial resolution is a key ingredient for the measurement and we provide a Gaussian parametrisation of the adaptive optics-assisted point spread function (PSF) for various wavelengths. From the MUSE data, we extracted the stellar kinematics and constructed dynamical models. Using an axisymmetric Schwarzschild technique, we measured an MBH of (3.6+2.7-2.4)\times 10^8 Msun at 3\sigma significance taking kinematical and dynamical systematics (e.g.,radially-varying mass-to-light ratio) into account. We also added a dark halo, but our data does not allow to constrain the dark matter fraction. Adding dark matter with an abundance matching prior results in a 25 per cent more massive black hole. Jeans anisotropic models return MBH of (4.6+2.5-2.7) \times 10^8 Msun and (8.6+0.8-0.8) \times 10^8 Msun at 3\sigma confidence for spherical and cylindrical alignment of the velocity ellipsoid, respectively. In a follow-up study, we will compare the stellar-based MBH with those from cold and warm gas tracers, which will provide additional constraints for the MBH for NGC 6958, and insights into assumptions that lead to potential systematic uncertainty.

==> papers <==
% This file was created with JabRef 2.10b2.
% Encoding: UTF8


@Article{Antonini2015,
  Title                    = {{The Coevolution of Nuclear Star Clusters, Massive Black Holes, and Their Host Galaxies}},
  Author                   = {{Antonini}, F. and {Barausse}, E. and {Silk}, J.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = oct,
  Pages                    = {72},
  Volume                   = {812},

  Abstract                 = {Studying how nuclear star clusters (NSCs) form and how they are related to the growth of the central massive black holes (MBHs) and their host galaxies is fundamental for our understanding of the evolution of galaxies and the processes that have shaped their central structures. We present the results of a semi-analytical galaxy formation model that follows the evolution of dark matter halos along merger trees, as well as that of the baryonic components. This model allows us to study the evolution of NSCs in a cosmological context, by taking into account the growth of NSCs due to both dynamical-friction-driven migration of stellar clusters and star formation triggered by infalling gas, while also accounting for dynamical heating from (binary) MBHs. We find that in situ star formation contributes a significant fraction (up to ∼80%) of the total mass of NSCs in our model. Both NSC growth through in situ star formation and that through star cluster migration are found to generate NSC—host galaxy scaling correlations that are shallower than the same correlations for MBHs. We explore the role of galaxy mergers on the evolution of NSCs and show that observational data on NSC—host galaxy scaling relations provide evidence of partial erosion of NSCs by MBH binaries in luminous galaxies. We show that this observational feature is reproduced by our models, and we make predictions about the NSC and MBH occupation fraction in galaxies. We conclude by discussing several implications for theories of NSC formation.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...812...72A},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/812/1/72},
  Eid                      = {72},
  Eprint                   = {1506.02050},
  Keywords                 = {galaxies: evolution, galaxies: formation, galaxies: nuclei, Galaxy: center, quasars: supermassive black holes},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Brok2015,
  Title                    = {MEASURING THE MASS OF THE CENTRAL BLACK HOLE IN THE BULGELESS GALAXY NGC 4395~{F}{ROM} GAS DYNAMICAL MODELING},
  Author                   = {Brok, Mark den and Seth, Anil C. and Barth, Aaron J. and Carson, Daniel J. and Neumayer, Nadine and Cappellari, Michele and Debattista, Victor P. and Ho, Luis C. and Hood, Carol E. and McDermid, Richard M.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2015},

  Month                    = {Aug},
  Number                   = {1},
  Pages                    = {101},
  Volume                   = {809},

  Comment                  = {Low mass BH},
  Doi                      = {10.1088/0004-637x/809/1/101},
  File                     = {Published version:Brok2015.pdf:PDF},
  ISSN                     = {1538-4357},
  Keywords                 = {NIFS, NGC 4395},
  Owner                    = {sinead},
  Publisher                = {IOP Publishing},
  Timestamp                = {2015.12.14},
  Url                      = {http://dx.doi.org/10.1088/0004-637X/809/1/101}
}

@Article{Cappellari2016,
  Title                    = {Structure and Kinematics of Early-Type Galaxies from Integral-Field Spectroscopy},
  Author                   = {Michele Cappellari},
  Year                     = {2016},

  Month                    = feb,
  Abstract                 = {Observations of galaxy isophotes, longs-slit kinematics and high-resolution photometry suggested a possible dichotomy between two distinct classes of E galaxies. But these methods are expensive for large galaxy samples. Instead, integral-field spectroscopic can efficiently recognize the shape, dynamics and stellar population of complete samples of early-type galaxies (ETGs). These studies showed that the two main classes, the fast and slow rotators, can be separated using stellar kinematics. We showed there is a dichotomy in the dynamics of the two classes. The slow rotators are weakly triaxial and dominate above $M_{\rm crit}\approx2\times10^{11} M_\odot$. Below $M_{\rm crit}$, the structure of fast rotators parallels that of spiral galaxies. There is a smooth sequence along which, the metals content, the enhancement in $\alpha$-elements, and the "weight" of the stellar initial mass function, all increase with the CENTRAL mass density slope, or bulge mass fraction, while the molecular gas fraction correspondingly decreases. The properties of ETGs on galaxy scaling relations, and in particular the $(M_{\ast}, R_{\rm e})$ diagram, and their dependence on environment, indicate two main independent channels for galaxy evolution. Fast rotators ETGs start as star forming disks and evolve trough a channel dominated by gas accretion, bulge growth and quenching. While slow rotators assemble near the center of massive halos via intense star formation at high redshift, and remain as such for the rest of their evolution via a channel dominated by gas poor mergers. This is consistent with independent studies of the galaxies redshift evolution.},
  Comments                 = {67 pages, 30 figures, LaTeX. To appear in Annual Review of Astronomy and Astrophysics (ARA&A), Vol. 54 (2016)},
  Eprint                   = {1602.04267},
  Oai2identifier           = {1602.04267},
  Owner                    = {sinead},
  Timestamp                = {2016.02.18}
}

@Article{Cappellari2008,
  Title                    = {{Measuring the inclination and mass-to-light ratio of axisymmetric galaxies via anisotropic Jeans models of stellar kinematics}},
  Author                   = {{Cappellari}, M.},
  Journal                  = {\mnras},
  Year                     = {2008},

  Month                    = oct,
  Pages                    = {71-86},
  Volume                   = {390},

  Abstract                 = {We present a simple and efficient anisotropic generalization of the semi-isotropic (two-integral) axisymmetric Jeans formalism, which is used to model the stellar kinematics of galaxies. The following is assumed: (i) a constant mass-to-light ratio (M/L) and (ii) a velocity ellipsoid that is aligned with cylindrical coordinates (R, z) and characterized by the classic anisotropy parameter . Our simple models are fit to SAURON integral-field observations of the stellar kinematics for a set of fast-rotator early-type galaxies. With only two free parameters (βz and the inclination), the models generally provide remarkably good descriptions of the shape of the first (V) and second () velocity moments, once a detailed description of the surface brightness is given. This is consistent with previous findings on the dynamical structure of these objects. With the observationally motivated assumption that βz >~ 0, the method is able to recover the inclination. The technique can be used to determine the dynamical M/L and angular momenta of early-type fast-rotators and spiral galaxies, especially when the quality of the data does not justify more sophisticated modelling approaches. This formalism allows for the inclusion of dark matter, supermassive black holes, spatially varying anisotropy and multiple kinematic components.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008MNRAS.390...71C},
  Archiveprefix            = {arXiv},
  Comment                  = {JAM},
  Doi                      = {10.1111/j.1365-2966.2008.13754.x},
  Eprint                   = {0806.0042},
  Keywords                 = {galaxies: elliptical and lenticular, cD , galaxies: evolution , galaxies: formation , galaxies: kinematics and dynamics , galaxies: structure},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Cappellari2002,
  Title                    = {Efficient multi-{Gauss}ian expansion of galaxies},
  Author                   = {Cappellari, M.},
  Journal                  = {Monthly Notices of the Royal Astronomical Society},
  Year                     = {2002},

  Month                    = {Jun},
  Number                   = {2},
  Pages                    = {400–410},
  Volume                   = {333},

  Comment                  = {MGE},
  Doi                      = {10.1046/j.1365-8711.2002.05412.x},
  File                     = {Published version:Cappellari2002.pdf:PDF},
  ISSN                     = {1365-2966},
  Keywords                 = {MGE},
  Owner                    = {sinead},
  Publisher                = {Oxford University Press (OUP)},
  Timestamp                = {2015.12.11},
  Url                      = {http://dx.doi.org/10.1046/j.1365-8711.2002.05412.x}
}

@Article{Cappellari2003,
  Title                    = {{Adaptive spatial binning of integral-field spectroscopic data using Voronoi tessellations}},
  Author                   = {{Cappellari}, M. and {Copin}, Y.},
  Journal                  = {\mnras},
  Year                     = {2003},

  Month                    = jun,
  Pages                    = {345-354},
  Volume                   = {342},

  Abstract                 = {We present new techniques to perform adaptive spatial binning of Integral-Field Spectroscopic (IFS) data to reach a chosen constant signal-to-noise ratio per bin. These methods are required for the proper analysis of IFS observations, but can also be used for standard photometric imagery or any other two-dimensional data. Various schemes are tested and compared by binning and extracting the stellar kinematics of the Sa galaxy NGC2273 from spectra obtained with the panoramic IFS SAURON.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2003MNRAS.342..345C},
  Comment                  = {Voronoi},
  Doi                      = {10.1046/j.1365-8711.2003.06541.x},
  Eprint                   = {astro-ph/0302262},
  Keywords                 = {methods: data analysis, techniques: photometric, techniques: spectroscopic},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Cappellari2009,
  Title                    = {{Dynamical Masses of Early-Type Galaxies at z \~{} 2: Are they Truly Superdense?}},
  Author                   = {{Cappellari}, M. and {di Serego Alighieri}, S. and {Cimatti}, A. and {Daddi}, E. and {Renzini}, A. and {Kurk}, J.~D. and {Cassata}, P. and {Dickinson}, M. and {Franceschini}, A. and {Mignoli}, M. and {Pozzetti}, L. and {Rodighiero}, G. and {Rosati}, P. and {Zamorani}, G. },
  Journal                  = {\apjl},
  Year                     = {2009},

  Month                    = oct,
  Pages                    = {L34-L39},
  Volume                   = {704},

  Abstract                 = {We measured stellar velocity dispersions σ and derived dynamical masses of nine massive (M ≈ 1011 M sun) early-type galaxies (ETGs) from the Galaxy Mass Assembly ultra-deep Spectroscopic Survey (GMASS) sample at redshift 1.4 lsim z lsim 2.0. The σ are based on individual spectra for two galaxies at z ≈ 1.4 and on a stacked spectrum for seven galaxies with 1.6 < z < 2.0, with 202 hr of exposure at the ESO Very Large Telescope. We constructed detailed axisymmetric dynamical models for the objects, based on the Jeans equations, taking the observed surface brightness (from deep HST/ACS observations), point-spread function, and slit effects into account. Our dynamical masses M Jeans agree within lsim30% with virial estimates M vir = 5 × Reσ2/G, although the latter tend to be smaller. Our M Jeans also agrees within a factor lsim2 with the M pop previously derived using stellar population models and 11 bands photometry. This confirms that the galaxies are intrinsically massive. The inferred mass-to-light ratios (M/L) U in the very age-sensitive rest-frame U band are consistent with passive evolution in the past ~1 Gyr (formation redshift zf ~ 3). A "bottom-light" stellar initial mass function appears to be required to ensure close agreement between M Jeans and M pop at z ~ 2, as it does at z ~ 0. The GMASS ETGs are on average more dense than their local counterpart. However, a few percent of local ETGs of similar dynamical masses also have comparable σ and mass surface density Σ50 inside R e. Based on observations collected at the European Southern Observatory, Paranal, Chile, ESO Large Programs 173.A-0687.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009ApJ...704L..34C},
  Archiveprefix            = {arXiv},
  Comment                  = {JAM},
  Doi                      = {10.1088/0004-637X/704/1/L34},
  Eprint                   = {0906.3648},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: high-redshift},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.GA},
  Timestamp                = {2015.12.18}
}

@Article{Cappellari2004,
  Title                    = {{Parametric Recovery of Line-of-Sight Velocity Distributions from Absorption-Line Spectra of Galaxies via Penalized Likelihood}},
  Author                   = {{Cappellari}, M. and {Emsellem}, E.},
  Journal                  = {\pasp},
  Year                     = {2004},

  Month                    = feb,
  Pages                    = {138-147},
  Volume                   = {116},

  Abstract                 = {We investigate the accuracy of the parametric recovery of the line-of-sight velocity distribution (LOSVD) of the stars in a galaxy while working in pixel space. Problems appear when the data have a low signal-to-noise ratio or the observed LOSVD is not well sampled by the data. We propose a simple solution based on maximum penalized likelihood, and we apply it to the common situation in which the LOSVD is described by a Gauss-Hermite series. We compare different techniques by extracting the stellar kinematics from observations of the barred lenticular galaxy NGC 3384 obtained with the SAURON integral-field spectrograph.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2004PASP..116..138C},
  Comment                  = {PPXF},
  Doi                      = {10.1086/381875},
  Eprint                   = {astro-ph/0312201},
  Keywords                 = {Galaxies: Individual: NGC Number: NGC 3384, Galaxies: Kinematics and Dynamics, line: profiles, Methods: Numerical},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Cappellari2002a,
  Title                    = {The Counterrotating Core and the Black Hole Mass of {IC} 1459},
  Author                   = {Cappellari, M. and Verolme, E. K. and van der Marel, R. P. and Kleijn, G. A. Verdoes and Illingworth, G. D. and Franx, M. and Carollo, C. M. and de Zeeuw, P. T.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2002},

  Month                    = {Oct},
  Number                   = {2},
  Pages                    = {787–805},
  Volume                   = {578},

  Doi                      = {10.1086/342653},
  ISSN                     = {1538-4357},
  Keywords                 = {IC 1459},
  Owner                    = {sinead},
  Publisher                = {IOP Publishing},
  Timestamp                = {2015.12.11},
  Url                      = {http://dx.doi.org/10.1086/342653}
}

@Article{Cappellari2002b,
  Title                    = {{The Counterrotating Core and the Black Hole Mass of IC 1459}},
  Author                   = {{Cappellari}, M. and {Verolme}, E.~K. and {van der Marel}, R.~P. and {Verdoes Kleijn}, G.~A. and {Illingworth}, G.~D. and {Franx}, M. and {Carollo}, C.~M. and {de Zeeuw}, P.~T.},
  Journal                  = {\apj},
  Year                     = {2002},

  Month                    = oct,
  Pages                    = {787-805},
  Volume                   = {578},

  Abstract                 = {The E3 giant elliptical galaxy IC 1459 is the prototypical galaxy with a fast counterrotating stellar core. We obtained one Hubble Space Telescope (HST) Space Telescope Imaging Spectrograph (STIS) long-slit spectrum along the major axis of this galaxy and Cerro Tololo Inter-American Observatory (CTIO) spectra along five position angles. The signal-to-noise ratio (S/N) of the ground-based data is such that also the higher order Gauss-Hermite moments (h3-h6) can be extracted reliably. We present self-consistent three-integral axisymmetric models of the stellar kinematics, obtained with Schwarzschild's numerical orbit superposition method. The available data allow us to study the dynamics of the kinematically decoupled core (KDC) in IC 1459, and we find that it consists of stars that are well separated from the rest of the galaxy in phase space. In particular, our study indicates that the stars in the KDC counterrotate in a disk on orbits that are close to circular. We estimate that the KDC mass is ~0.5% of the total galaxy mass or ~3×109 Msolar. We estimate the central black hole (BH) mass MBH of IC 1459 independently from both its stellar and its gaseous kinematics. Although both tracers rule out models without a central BH, neither yields a particularly accurate determination of the BH mass. The main problem for the stellar dynamical modeling is the fact that the modest S/N of the STIS spectrum and the presence of strong gas emission lines preclude measuring the full line-of-sight velocity distribution (LOSVD) at HST resolution. The main problem for the gasdynamical modeling is that there is evidence that the gas motions are disturbed, possibly as a result of nongravitational forces acting on the gas. These complications probably explain why we find rather discrepant BH masses with the different methods. The stellar kinematics suggest that MBH=(2.6+/-1.1)×109 Msolar (3 σ error). The gas kinematics suggests that MBH~3.5×108 Msolar if the gas is assumed to rotate at the circular velocity in a thin disk. If the observed velocity dispersion of the gas is assumed to be gravitational, then MBH could be as high as ~1.0×109 Msolar. These different estimates bracket the value MBH=(1.1+/-0.3)×109 Msolar predicted by the MBH-σ relation. It will be an important goal for future studies to attempt comparisons of BH mass determinations from stellar and gaseous kinematics for other galaxies. This will assess the reliability of BH mass determinations with either technique. This is essential if one wants to interpret the correlation between the BH mass and other global galaxy parameters (e.g., velocity dispersion) and in particular the scatter in these correlations (believed to be only ~0.3 dex). Based on observations with the NASA/ESA Hubble Space Telescope obtained at the Space Telescope Science Institute, which is operated by AURA, Inc., under NASA contract NAS 5-26555. These observations are associated with proposal 7352.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2002ApJ...578..787C},
  Comment                  = {dust correction},
  Doi                      = {10.1086/342653},
  Eprint                   = {astro-ph/0202155},
  Keywords                 = {Black Hole Physics, Galaxies: Elliptical and Lenticular, cD, Galaxies: Individual: Alphanumeric: IC 1459, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Carollo1997a,
  Title                    = {{Ellipticals with Kinematically Distinct Cores: V - I Color Images with WPFC2}},
  Author                   = {{Carollo}, C.~M. and {Franx}, M. and {Illingworth}, G.~D. and {Forbes}, D.~A.},
  Journal                  = {\apj},
  Year                     = {1997},

  Month                    = may,
  Pages                    = {710-734},
  Volume                   = {481},

  Abstract                 = {We have analyzed Hubble Space Telescope WFPC2 F555W and F814W (i.e., V and I) images for 15 elliptical galaxies with kinematically distinct cores. For each of them, we have derived surface brightness and isophotal parameter profiles in the two bands, color maps, and radial profiles in V - I. Most galaxies show patchy dust absorption close to their nuclei. However, there are generally no indications of homogeneous, diffuse dust components close to the nuclei. The nuclear colors in the unobscured regions are most likely representative of the central stellar populations. We have detected photometric evidence for faint stellar disks, on scales of a few tens to a few arcseconds, in seven galaxies, namely NGC 1427, 1439, 1700, 4365, 4406, 4494, and 5322. In NGC 1700, the isophotes are slightly boxy at the scale of the counterrotating component and disky at larger radii. We find no difference in V - I color greater than 0.02 mag between these disks and the surrounding galactic regions. Hence, the stellar populations in the kinematically distinct cores are not strongly deviant from the population of the main body. Specifically, there is no evidence for a dominating population of blue, very metal weak stars as predicted by some of the formation scenarios. This argues against models in which small galaxies fall in and survive in the nuclei, unless supermassive black holes are present. These would likely disrupt the accreted small systems. For one galaxy, NGC 4365, the innermost region is bluer than the surrounding regions. This area extends to ~15 pc and contains a luminosity of ~2.5 × 106 L⊙. If interpreted as a stellar population effect, an age difference of ~3-4 Gyr, or an [Fe/H] variation of about 0.2 dex, is derived. The nuclear intensity profiles show a large variety: some galaxies have steep cusp profiles, while others have shallow cusps and a ``break radius.'' The nuclear cusps of galaxies with kinematically distinct cores follow the same trends as the nuclei of normal galaxies. We have not been able to identify a unique, qualifying feature in the WFPC2 images that distinguishes the galaxies with kinematically distinct cores from the kinematically normal cores. It is possible that statistical differences exist: possibly, the kinematically distinct cores have a higher fraction of nuclear disks. The similarity of both types of cores puts strong constraints on the formation scenarios. Simulations of galaxy mergers, with the inclusion of star formation and nuclear black holes, are needed to resolve the question of how these structures may have formed. Spectra with high spatial resolution are needed to study the nuclear structure of the distinct component in detail. Based on observations with the NASA/ESA Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by Association of Universities for Research in Astronomy, Inc. (AURA), under NASA contract NAS 5-26555.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/1997ApJ...481..710C},
  Comment                  = {dust correction},
  Eprint                   = {astro-ph/9701218},
  Keywords                 = {Galaxies: Elliptical and Lenticular, cD, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Photometry, Galaxies: Stellar Content},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Cole2016,
  Title                    = {{Nuclear Star Clusters and Bulges}},
  Author                   = {{Cole}, D.~R. and {Debattista}, V.~P.},
  Journal                  = {Galactic Bulges},
  Year                     = {2016},
  Pages                    = {107},
  Volume                   = {418},
  Abstract                 = {Nuclear star clusters are among the densest stellar systems known and are common in both early- and late-type galaxies. They exhibit scaling relations with their host galaxy which may be related to those of supermassive black holes (SMBHs). These may therefore help us to unravel the complex physical processes occurring at the centers of galaxies. The properties of nuclear stellar systems suggest that their formation requires both dissipational and dissipationless processes. They have stellar populations of different ages, from stars as old as their host galaxy to young stars formed in the last 100 Myr. Therefore star formation must be happening either directly in the nuclear star cluster or in its vicinity. The secular processes that fuel the formation of pseudobulges very likely also contribute to nuclear star cluster growth.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016ASSL..418..107C},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1007/978-3-319-19378-6_5},
  Eprint                   = {1504.05879},
  File                     = {arXiv v1:Cole2016-eprintv1.pdf:PDF},
  Keywords                 = {Physics},
  Owner                    = {sinead},
  Timestamp                = {2016.02.16}
}

@Article{Cretton1999,
  Title                    = {Evidence for a Massive Black Hole in the S0 Galaxy NGC 4342},
  Author                   = {Cretton, Nicolas and van den Bosch, Frank C.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {1999},

  Month                    = {Apr},
  Number                   = {2},
  Pages                    = {704–724},
  Volume                   = {514},

  Doi                      = {10.1086/306971},
  ISSN                     = {1538-4357},
  Keywords                 = {NGC 4342},
  Owner                    = {sinead},
  Publisher                = {IOP Publishing},
  Timestamp                = {2015.12.11},
  Url                      = {http://dx.doi.org/10.1086/306971}
}

@Article{deBlok2014,
  Title                    = {{HALOGAS observations of NGC 4414: fountains, interaction, and ram pressure}},
  Author                   = {{de Blok}, W.~J.~G. and {J{\'o}zsa}, G.~I.~G. and {Patterson}, M. and {Gentile}, G. and {Heald}, G.~H. and {J{\"u}tte}, E. and {Kamphuis}, P. and {Rand}, R.~J. and {Serra}, P. and {Walterbos}, R.~A.~M.},
  Journal                  = {\aap},
  Year                     = {2014},

  Month                    = jun,
  Pages                    = {A80},
  Volume                   = {566},

  Abstract                 = {We present deep H i imaging of the nearby spiral galaxy NGC 4414, taken as part of the Westerbork HALOGAS (Hydrogen Accretion in LOcal GAlaxieS) survey. The observations show that NGC 4414 can be characterized by a regularly rotating inner H i disk, and a more disturbed outer disk. Modeling of the kinematics shows that the outer disk is best described by a U-shaped warp. Deep optical imaging also reveals the presence of a low surface brightness stellar shell, indicating a minor interaction with a dwarf galaxy at some stage in the past. Modeling of the inner disk suggests that about 4 percent of the inner H i is in the form of extra-planar gas. Because of the disturbed nature of the outer disk, this number is difficult to constrain for the galaxy as a whole. These new, deep observations of NGC 4414 presented here show that even apparently undisturbed galaxies are interacting with their environment.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2014A%26A...566A..80D},
  Archiveprefix            = {arXiv},
  Comment                  = {SFR=4.2 M/a, minor interaction, outer disk shows disturbances},
  Doi                      = {10.1051/0004-6361/201322517},
  Eid                      = {A80},
  Eprint                   = {1405.2160},
  File                     = {Published version:deBlok2014.pdf:PDF},
  Keywords                 = {NGC 4414},
  Owner                    = {sinead},
  Timestamp                = {2015.12.15}
}

@Article{Do2014,
  Title                    = {{Prospects for Measuring Supermassive Black Hole Masses with Future Extremely Large Telescopes}},
  Author                   = {{Do}, T. and {Wright}, S.~A. and {Barth}, A.~J. and {Barton}, E.~J. and {Simard}, L. and {Larkin}, J.~E. and {Moore}, A.~M. and {Wang}, L. and {Ellerbroek}, B.},
  Journal                  = {\aj},
  Year                     = {2014},

  Month                    = apr,
  Pages                    = {93},
  Volume                   = {147},

  Abstract                 = {The next generation of giant-segmented mirror telescopes (>20 m) will enable us to observe galactic nuclei at much higher angular resolution and sensitivity than ever before. These capabilities will introduce a revolutionary shift in our understanding of the origin and evolution of supermassive black holes by enabling more precise black hole mass measurements in a mass range that is unreachable today. We present simulations and predictions of the observations of nuclei that will be made with the Thirty Meter Telescope (TMT) and the adaptive optics assisted integral-field spectrograph IRIS, which is capable of diffraction-limited spectroscopy from Z band (0.9 μm) to K band (2.2 μm). These simulations, for the first time, use realistic values for the sky, telescope, adaptive optics system, and instrument to determine the expected signal-to-noise ratio of a range of possible targets spanning intermediate mass black holes of ~104 M ⊙ to the most massive black holes known today of >1010 M ⊙. We find that IRIS will be able to observe Milky Way mass black holes out the distance of the Virgo Cluster, and will allow us to observe many more of the brightest cluster galaxies where the most massive black holes are thought to reside. We also evaluate how well the kinematic moments of the velocity distributions can be constrained at the different spectral resolutions and plate scales designed for IRIS. We find that a spectral resolution of ~8000 will be necessary to measure the masses of intermediate mass black holes. By simulating the observations of galaxies found in Sloan Digital Sky Survey DR7, we find that over 105 massive black holes will be observable at distances between 0.005 < z < 0.18 with the estimated sensitivity and angular resolution provided by access to Z-band (0.9 μm) spectroscopy from IRIS and the TMT adaptive optics system. These observations will provide the most accurate dynamical measurements of black hole masses to enable the study of the demography of massive black holes, address the origin of the M BH - σ and M BH - L relationships, and evolution of black holes through cosmic time.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2014AJ....147...93D},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-6256/147/4/93},
  Eid                      = {93},
  Eprint                   = {1401.7988},
  Keywords                 = {galaxies: kinematics and dynamics, instrumentation: adaptive optics, instrumentation: spectrographs, techniques: imaging spectroscopy, telescopes},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Drehmer2015,
  Title                    = {{The benchmark black hole in NGC 4258: dynamical models from high-resolution two-dimensional stellar kinematics}},
  Author                   = {{Drehmer}, D.~A. and {Storchi-Bergmann}, T. and {Ferrari}, F. and {Cappellari}, M. and {Riffel}, R.~A.},
  Journal                  = {\mnras},
  Year                     = {2015},

  Month                    = jun,
  Pages                    = {128-144},
  Volume                   = {450},

  Abstract                 = {NGC 4258 is the galaxy with the most accurate (maser-based) determination for the mass of the supermassive black hole (SMBH) in its nucleus. In this work, we present a two-dimensional mapping of the stellar kinematics in the inner 3.0 arcsec × 3.0 arcsec = 100 pc × 100 pc of NGC 4258 using adaptive-optics observations obtained with the Near-Infrared Integral Field Spectrograph of the Gemini North telescope at an ≈0.11 arcsec (4 pc) angular resolution. The observations resolve the radius of influence of the SMBH, revealing an abrupt increase in the stellar velocity dispersion within ≈10 pc from the nucleus, consistent with the presence of an SMBH there. Assuming that the galaxy nucleus is in a steady state and that the velocity dispersion ellipsoid is aligned with a cylindrical coordinate system, we constructed a Jeans anisotropic dynamical model to fit the observed kinematics distribution. Our dynamical model assumes that the galaxy has axial symmetry and is constructed using the multi-Gaussian expansion method to parametrize the observed surface brightness distribution. The Jeans dynamical model has three free parameters: the mass of the central SMBH (M•), the mass-luminosity ratio (Γk = M/L) of the galaxy and the anisotropy of the velocity distribution. We test two types of models: one with constant velocity anisotropy, and another with variable anisotropy. The model that best reproduces the observed kinematics was obtained considering that the galaxy has radially varying anisotropy, being the best-fitting parameters with 3σ significance M_bullet =4.8^{+0.8}_{-0.9}× 10^7 {M_{⊙}} and Γ _k = 4.1^{+0.4}_{-0.5}. This value for the mass of the SMBH is just 25 per cent larger than that of the maser determination and 50 per cent larger that a previous stellar dynamical determination obtained via Schwarzschild models for long-slit data that provides an SMBH mass 15 per cent lower than the maser value.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015MNRAS.450..128D},
  Archiveprefix            = {arXiv},
  Comment                  = {Davor Empfehlung},
  Doi                      = {10.1093/mnras/stv536},
  Eprint                   = {1503.04540},
  File                     = {Published version:Drehmer2015.pdf:PDF},
  Keywords                 = {galaxies: individual: NGC 4258, galaxies: kinematics and dynaNIFS, JAM, NIFS},
  Owner                    = {sinead},
  Timestamp                = {2016.01.05}
}

@Article{Falcon-Barroso2011,
  Title                    = {{An updated MILES stellar library and stellar population models}},
  Author                   = {{Falc{\'o}n-Barroso}, J. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Vazdekis}, A. and {Ricciardelli}, E. and {Cardiel}, N. and {Cenarro}, A.~J. and {Gorgas}, J. and {Peletier}, R.~F.},
  Journal                  = {\aap},
  Year                     = {2011},

  Month                    = aug,
  Pages                    = {A95},
  Volume                   = {532},

  __markedentry            = {[sinead:6]},
  Abstract                 = { Aims: We present a number of improvements to the MILES library and stellar population models. We correct some small errors in the radial velocities of the stars, measure the spectral resolution of the library and models more accurately, and give a better absolute flux calibration of the models.  Methods: We use cross-correlation techniques to correct the radial velocities of the offset stars and the penalised pixel-fitting method, together with different sets of stellar templates, to re-assess the spectral resolution of the MILES stellar library and models. We have also re-calibrated the zero-point flux level of the models using a new calibration scheme.  Results: The end result is an even more homogeneously calibrated stellar library than the originally released one, with a measured spectral resolution of ~2.5 Å, almost constant with wavelength, for both the MILES stellar library and models. Furthermore, the new absolute flux calibration for the spectra excellently agrees with predictions based on independent photometric libraries.  Conclusions: This improved version of the MILES library and models (version 9.1) is available at the project's website (http://miles.iac.es).},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011A%26A...532A..95F},
  Archiveprefix            = {arXiv},
  Comment                  = {MILES},
  Doi                      = {10.1051/0004-6361/201116842},
  Eid                      = {A95},
  Eprint                   = {1107.2303},
  Keywords                 = {catalogs, methods: data analysis, techniques: spectroscopic, stars: kinematics and dynamics, galaxies: kinematics and dynamics},
  Owner                    = {sinead},
  Timestamp                = {2016.02.18}
}

@Article{Ferre-Mateu2015,
  Title                    = {{Massive Relic Galaxies Challenge the Co-evolution of Super-massive Black Holes and Their Host Galaxies}},
  Author                   = {{Ferr{\'e}-Mateu}, A. and {Mezcua}, M. and {Trujillo}, I. and {Balcells}, M. and {van den Bosch}, R.~C.~E.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = jul,
  Pages                    = {79},
  Volume                   = {808},

  Abstract                 = {We study a sample of eight massive galaxies that are extreme outliers (3-5σ) in the {M}\bullet - Mbulge local scaling relation. Two of these galaxies are confirmed to host extremely large super-massive black holes (SMBHs), whereas the virial mass estimates for the other six are also consistent with having abnormally large SMBHs. From the analysis of their star formation histories and their structural properties, we find that all of these extreme outliers can be considered to be relic galaxies from the early (z ˜ 2) universe: i.e., they are compact (R {}{{e}}\lt 2 kpc) and have purely old stellar populations (t≳ 10 Gyr). In order to explain the nature of such deviations from the local relations, we propose a scenario in which the hosts of these über-massive SMBHs are galaxies that have followed a different evolutionary path than the two-phase growth channel assumed for massive galaxies. Once the SMBH and the core of the galaxy are formed at z ˜ 2, the galaxy skips the second phase, remaining structurally untouched and without further mass and size increase. We show that if the outliers had followed the normal evolutionary path by growing in size via merger activity, the expected (mild) growth in mass would place them closer to the observed local relations. Our results suggest that the SMBH growth epoch for the most massive galaxies stopped ˜10 Gyr ago.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...808...79F},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/808/1/79},
  Eid                      = {79},
  Eprint                   = {1506.02663},
  Keywords                 = {accretion, accretion disks, black hole physics, galaxies: evolution, galaxies: formation, galaxies: nuclei, galaxies: stellar content},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Fisher2009,
  Title                    = {{Bulges of Nearby Galaxies with Spitzer: The Growth of Pseudobulges in Disk Galaxies and its Connection to Outer Disks}},
  Author                   = {{Fisher}, D.~B. and {Drory}, N. and {Fabricius}, M.~H.},
  Journal                  = {\apj},
  Year                     = {2009},

  Month                    = may,
  Pages                    = {630-650},
  Volume                   = {697},

  Abstract                 = {We study star formation rates (SFRs) and stellar masses in bulges of nearby disk galaxies. For this we construct a new SFR indicator that linearly combines data from the Spitzer Space Telescope and the Galaxy Evolution Explorer. All bulges are found to be forming stars irrespective of bulge type (pseudobulge or classical bulge). At present-day SFR the median pseudobulge could have grown the present-day stellar mass in 8 Gyr. Classical bulges have the lowest specific SFR implying a growth times that are longer than a Hubble time, and thus the present-day SFR does not likely play a major role in the evolution of classical bulges. In almost all galaxies in our sample the specific SFR (SFR per unit stellar mass) of the bulge is higher than that of the outer disk. This suggests that almost all galaxies are increasing their B/T through internal star formation. The SFR in pseudobulges correlates with their structure. More massive pseudobulges have higher SFR density, this is consistent with that stellar mass being formed by moderate, extended star formation. Bulges in late-type galaxies have similar SFRs as pseudobulges in intermediate-type galaxies, and are similar in radial size. However, they are deficient in mass; thus, they have much shorter growth times, ~2 Gyr. We identify a class of bulges that have nuclear morphology similar to pseudobulges, significantly lower specific SFR than pseudobulges, and are closer to classical bulges in structural parameter correlations. These are possibly composite objects, evolved pseudobulges or classical bulges experiencing transient, enhanced nuclear star formation. Our results are consistent with a scenario in which bulge growth via internal star formation is a natural, and near ubiquitous phenomenon in disk galaxies. Those galaxies with large classical bulges are not affected by the in situ bulge growth, likely because the majority of their stellar mass comes from some other phenomenon. Yet, those galaxies without a classical bulge, over long periods of extended star formation are able to growth a pseudobulge. Though cold accretion is not ruled out, for pseudobulge galaxies an addition of stellar mass from mergers or accretion is not required to explain the bulge mass. In this sense, galaxies with pseudobulges may very well be bulgeless (or "quasi-bulgeless") galaxies, and galaxies with classical bulges are galaxies in which both internal evolution and hierarchical merging are responsible for the bulge mass by fractions that vary from galaxy to galaxy.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009ApJ...697..630F},
  Archiveprefix            = {arXiv},
  Comment                  = {Pseudobulge},
  Doi                      = {10.1088/0004-637X/697/1/630},
  Eprint                   = {0902.3258},
  File                     = {Published version:Fisher2009.pdf:PDF},
  Keywords                 = {galaxies: bulges, galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: structure},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.CO},
  Timestamp                = {2015.12.15}
}

@Article{Fontanot2015,
  Title                    = {{Interpreting the possible break in the black hole-bulge mass relation}},
  Author                   = {{Fontanot}, F. and {Monaco}, P. and {Shankar}, F.},
  Journal                  = {\mnras},
  Year                     = {2015},

  Month                    = nov,
  Pages                    = {4112-4120},
  Volume                   = {453},

  Abstract                 = {Recent inspections of local available data suggest that the almost linear relation between the stellar mass of spheroids (Msph) and the mass of the super massive black holes (BHs), residing at their centres, shows a break below Msph ˜ 1010 M⊙, with a steeper, about quadratic relation at smaller masses. We investigate the physical mechanisms responsible for the change in slope of this relation, by comparing data with the results of the semi-analytic model of galaxy formation MORGANA, which already predicted such a break in its original formulation. We find that the change of slope is mostly induced by effective stellar feedback in star-forming bulges. The shape of the relation is instead quite insensitive to other physical mechanisms connected to BH accretion such as disc instabilities, galaxy mergers, active galactic nucleus (AGN) feedback, or even the exact modelling of accretion on to the BH, direct or through a reservoir of low angular momentum gas. Our results support a scenario where most stars form in the disc component of galaxies and are carried to bulges through mergers and disc instabilities, while accretion on to BHs is connected to star formation in the spheroidal component. Therefore, a model of stellar feedback that produces stronger outflows in star-forming bulges than in discs will naturally produce a break in the scaling relation. Our results point to a form of co-evolution especially at lower masses, below the putative break, mainly driven by stellar feedback rather than AGN feedback.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015MNRAS.453.4112F},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stv1930},
  Eprint                   = {1508.06997},
  Keywords                 = {galaxies: active, galaxies: bulges, galaxies: evolution},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Freudling2013,
  Title                    = {{Automated data reduction workflows for astronomy. The ESO Reflex environment}},
  Author                   = {{Freudling}, W. and {Romaniello}, M. and {Bramich}, D.~M. and {Ballester}, P. and {Forchi}, V. and {Garc{\'{\i}}a-Dabl{\'o}}, C.~E. and {Moehler}, S. and {Neeser}, M.~J.},
  Journal                  = {\aap},
  Year                     = {2013},

  Month                    = nov,
  Pages                    = {A96},
  Volume                   = {559},

  Abstract                 = {Context. Data from complex modern astronomical instruments often consist of a large number of different science and calibration files, and their reduction requires a variety of software tools. The execution chain of the tools represents a complex workflow that needs to be tuned and supervised, often by individual researchers that are not necessarily experts for any specific instrument. Aims: The efficiency of data reduction can be improved by using automatic workflows to organise data and execute a sequence of data reduction steps. To realize such efficiency gains, we designed a system that allows intuitive representation, execution and modification of the data reduction workflow, and has facilities for inspection and interaction with the data. Methods: The European Southern Observatory (ESO) has developed Reflex, an environment to automate data reduction workflows. Reflex is implemented as a package of customized components for the Kepler workflow engine. Kepler provides the graphical user interface to create an executable flowchart-like representation of the data reduction process. Key features of Reflex are a rule-based data organiser, infrastructure to re-use results, thorough book-keeping, data progeny tracking, interactive user interfaces, and a novel concept to exploit information created during data organisation for the workflow execution. Results: Automated workflows can greatly increase the efficiency of astronomical data reduction. In Reflex, workflows can be run non-interactively as a first step. Subsequent optimization can then be carried out while transparently re-using all unchanged intermediate products. We found that such workflows enable the reduction of complex data by non-expert users and minimizes mistakes due to book-keeping errors. Conclusions: Reflex includes novel concepts to increase the efficiency of astronomical data processing. While Reflex is a specific implementation of astronomical scientific workflows within the Kepler workflow engine, the overall design choices and methods can also be applied to other environments for running automated science workflows.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2013A%26A...559A..96F},
  Archiveprefix            = {arXiv},
  Comment                  = {Reflex, SINFONI},
  Doi                      = {10.1051/0004-6361/201322494},
  Eid                      = {A96},
  Eprint                   = {1311.5411},
  Keywords                 = {methods: data analysis, astronomical databases: miscellaneous, techniques: miscellaneous, virtual observatory tools},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.IM},
  Timestamp                = {2015.12.18}
}

@Article{Gueltekin2009a,
  Title                    = {{A Quintet of Black Hole Mass Determinations}},
  Author                   = {{G{\"u}ltekin}, K. and {Richstone}, D.~O. and {Gebhardt}, K. and {Lauer}, T.~R. and {Pinkney}, J. and {Aller}, M.~C. and {Bender}, R. and {Dressler}, A. and {Faber}, S.~M. and {Filippenko}, A.~V. and {Green}, R. and {Ho}, L.~C. and {Kormendy}, J. and {Siopis}, C. },
  Journal                  = {\apj},
  Year                     = {2009},

  Month                    = apr,
  Pages                    = {1577-1590},
  Volume                   = {695},

  Abstract                 = {We report five new measurements of central black hole masses based on Space Telescope Imaging Spectrograph and Wide Field Planetary Camera 2 observations with the Hubble Space Telescope (HST) and on axisymmetric, three-integral, Schwarzschild orbit-library kinematic models. We selected a sample of galaxies within a narrow range in velocity dispersion that cover a range of galaxy parameters (including Hubble type and core/power-law surface density profile) where we expected to be able to resolve the galaxy's sphere of influence based on the predicted value of the black hole mass from the M-σ relation. We find masses for the following galaxies: NGC 3585, M BH = 3.4+1.5 -0.6 × 108 M sun; NGC 3607, M BH = 1.2+0.4 -0.4 × 108 M sun; NGC 4026, M BH = 2.1+0.7 -0.4 × 108 M sun; and NGC 5576, M BH = 1.8+0.3 -0.4 × 108 M sun, all significantly excluding M BH = 0. For NGC 3945, M BH = 9+17 -21 × 106 M sun, which is significantly below predictions from M-σ and M-L relations and consistent with M BH = 0, though the presence of a double bar in this galaxy may present problems for our axisymmetric code. Based on observations made with the Hubble Space Telescope, obtained at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555. These observations are associated with GO proposals 5999, 6587, 6633, 7468, and 9107.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009ApJ...695.1577G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/695/2/1577},
  Eprint                   = {0901.4162},
  Keywords                 = {black hole physics, galaxies: general, galaxies: nuclei, stellar dynamics},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.GA},
  Timestamp                = {2015.12.21}
}

@Article{Gueltekin2009,
  Title                    = {{The M-{$\sigma$} and M-L Relations in Galactic Bulges, and Determinations of Their Intrinsic Scatter}},
  Author                   = {{G{\"u}ltekin}, K. and {Richstone}, D.~O. and {Gebhardt}, K. and {Lauer}, T.~R. and {Tremaine}, S. and {Aller}, M.~C. and {Bender}, R. and {Dressler}, A. and {Faber}, S.~M. and {Filippenko}, A.~V. and {Green}, R. and {Ho}, L.~C. and {Kormendy}, J. and {Magorrian}, J. and {Pinkney}, J. and {Siopis}, C.},
  Journal                  = {\apj},
  Year                     = {2009},

  Month                    = jun,
  Pages                    = {198-221},
  Volume                   = {698},

  Abstract                 = {We derive improved versions of the relations between supermassive black hole mass (M BH) and host-galaxy bulge velocity dispersion (σ) and luminosity (L; the M-σ and M-L relations), based on 49 M BH measurements and 19 upper limits. Particular attention is paid to recovery of the intrinsic scatter (epsilon0) in both relations. We find log(M BH/M sun) = α + βlog(σ/200 km s-1) with (α, β, epsilon0) = (8.12 ± 0.08, 4.24 ± 0.41, 0.44 ± 0.06) for all galaxies and (α, β, epsilon0) = (8.23 ± 0.08, 3.96 ± 0.42, 0.31 ± 0.06) for ellipticals. The results for ellipticals are consistent with previous studies, but the intrinsic scatter recovered for spirals is significantly larger. The scatter inferred reinforces the need for its consideration when calculating local black hole mass function based on the M-σ relation, and further implies that there may be substantial selection bias in studies of the evolution of the M-σ relation. We estimate the M-L relationship as log(M BH/M sun) = α + βlog(LV /1011 L sun,V ) of (α, β, epsilon0) = (8.95 ± 0.11, 1.11 ± 0.18, 0.38 ± 0.09); using only early-type galaxies. These results appear to be insensitive to a wide range of assumptions about the measurement errors and the distribution of intrinsic scatter. We show that culling the sample according to the resolution of the black hole's sphere of influence biases the relations to larger mean masses, larger slopes, and incorrect intrinsic residuals.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009ApJ...698..198G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/698/1/198},
  Eprint                   = {0903.4897},
  Keywords                 = {black hole physics, galaxies: general, galaxies: nuclei, galaxies: statistics, stellar dynamics},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.GA},
  Timestamp                = {2015.12.21}
}

@Article{Gebhardt2011,
  Title                    = {{The Black Hole Mass in M87 from Gemini/NIFS Adaptive Optics Observations}},
  Author                   = {{Gebhardt}, K. and {Adams}, J. and {Richstone}, D. and {Lauer}, T.~R. and {Faber}, S.~M. and {G{\"u}ltekin}, K. and {Murphy}, J. and {Tremaine}, S. },
  Journal                  = {\apj},
  Year                     = {2011},

  Month                    = mar,
  Pages                    = {119},
  Volume                   = {729},

  Abstract                 = {We present the stellar kinematics in the central 2'' of the luminous elliptical galaxy M87 (NGC 4486), using laser adaptive optics to feed the Gemini telescope integral-field spectrograph, Near-infrared Integral Field Spectrograph (NIFS). The velocity dispersion rises to 480 km s-1 at 0farcs2. We combine these data with extensive stellar kinematics out to large radii to derive a black hole mass equal to (6.6 ± 0.4) × 109 M sun, using orbit-based axisymmetric models and including only the NIFS data in the central region. Including previously reported ground-based data in the central region drops the uncertainty to 0.25 × 109 M sun with no change in the best-fit mass; however, we rely on the values derived from the NIFS-only data in the central region in order to limit systematic differences. The best-fit model shows a significant increase in the tangential velocity anisotropy of stars orbiting in the central region with decreasing radius, similar to that seen at the centers of other core galaxies. The black hole mass is insensitive to the inclusion of a dark halo in the models—the high angular resolution provided by the adaptive optics breaks the degeneracy between black hole mass and stellar mass-to-light ratio. The present black hole mass is in excellent agreement with the Gebhardt & Thomas value, implying that the dark halo must be included when the kinematic influence of the black hole is poorly resolved. This degeneracy implies that the black hole masses of luminous core galaxies, where this effect is important, may need to be re-evaluated. The present value exceeds the prediction of the black hole-dispersion and black hole-luminosity relations, both of which predict about 1 × 109 M sun for M87, by close to twice the intrinsic scatter in the relations. The high end of the black hole correlations may be poorly determined at present.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011ApJ...729..119G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/729/2/119},
  Eid                      = {119},
  Eprint                   = {1101.1954},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: individual: M87 NGC 4486, galaxies: kinematics and dynamics},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{2016arXiv160102613G,
  Title                    = {{Masses and Scaling Relations for Nuclear Star Clusters, and their Coexistence with Central Black Holes}},
  Author                   = {{Georgiev}, I.~Y. and {B{\"o}ker}, T. and {Leigh}, N. and {L{\"u}tzgendorf}, N. and {Neumayer}, N.},
  Journal                  = {ArXiv e-prints},
  Year                     = {2016},

  Month                    = jan,

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016arXiv160102613G},
  Archiveprefix            = {arXiv},
  Eprint                   = {1601.02613},
  File                     = {arXiv v1:2016arXiv160102613G-eprintv1.pdf:PDF},
  Keywords                 = {Astrophysics - Astrophysics of Galaxies},
  Owner                    = {sinead},
  Timestamp                = {2016.01.18}
}

@Article{Gurovich2010,
  Title                    = {{The Slope of the Baryonic Tully-Fisher Relation}},
  Author                   = {{Gurovich}, S. and {Freeman}, K. and {Jerjen}, H. and {Staveley-Smith}, L. and {Puerari}, I.},
  Journal                  = {\aj},
  Year                     = {2010},

  Month                    = sep,
  Pages                    = {663-676},
  Volume                   = {140},

  Abstract                 = {We present the results of a baryonic Tully-Fisher relation (BTFR) study for a local sample of relatively isolated disk galaxies. We derive a BTFR with a slope near 3 measured over about 4 dex in baryon mass for our combined H I and bright spiral disk samples. This BTFR is significantly flatter and has less scatter than the TFR (stellar mass only) with its slope near 4 reported for other samples and studies. A BTFR slope near 3 is in better agreement with the expected slope from simple ΛCDM cosmological simulations that include both stellar and gas baryons. The scatter in the TFR/BTFR appears to depend on W 20: galaxies that rotate slower have more scatter. The atomic gas-to-stars ratio shows a break near W 20 = 250 km s-1 probably associated with a change in star formation efficiency. In contrast, the absence of such a break in the BTFR suggests that this relation was probably set at the main epoch of baryon dissipation rather than as a product of later galactic evolution.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2010AJ....140..663G},
  Archiveprefix            = {arXiv},
  Comment                  = {[Fe/H]=-0.08},
  Doi                      = {10.1088/0004-6256/140/3/663},
  Eprint                   = {1004.4365},
  Keywords                 = {cosmology: observations, dark matter, galaxies: evolution, galaxies: formation},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Heald2011,
  Title                    = {{The Westerbork Hydrogen Accretion in LOcal GAlaxieS (HALOGAS) survey. I. Survey description and pilot observations}},
  Author                   = {{Heald}, G. and {J{\'o}zsa}, G. and {Serra}, P. and {Zschaechner}, L. and {Rand}, R. and {Fraternali}, F. and {Oosterloo}, T. and {Walterbos}, R. and {J{\"u}tte}, E. and {Gentile}, G.},
  Journal                  = {\aap},
  Year                     = {2011},

  Month                    = feb,
  Pages                    = {A118},
  Volume                   = {526},

  Abstract                 = {We introduce a new, very deep neutral hydrogen (H i) survey being performed with the Westerbork Synthesis Radio Telescope (WSRT). The Westerbork Hydrogen Accretion in LOcal GAlaxieS (HALOGAS) Survey is producing an archive of some of the most sensitive H i observations available, on the angular scales which are most useful for studying faint, diffuse gas in and around nearby galaxies. The survey data are being used to perform careful modeling of the galaxies, characterizing their gas content, morphology, and kinematics, with the primary goal of revealing the global characteristics of cold gas accretion onto spiral galaxies in the local Universe. In this paper, we describe the survey sample selection, the data acquisition, reduction, and analysis, and present the data products obtained during our pilot program, which consists of UGC 2082, NGC 672, NGC 925, and NGC 4565. The observations reveal a first glimpse of the picture that the full HALOGAS project aims to illuminate: the properties of accreting H i in different types of spirals, and across a range of galactic environments. None of the pilot survey galaxies hosts an H i halo of the scale of NGC 891, but all show varying indications of halo gas features. We compare the properties of detected features in the pilot survey galaxies with their global characteristics, and discuss similarities and differences with NGC 891 and NGC 2403.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011A%26A...526A.118H},
  Archiveprefix            = {arXiv},
  Comment                  = {SFR=4.2 M/a},
  Doi                      = {10.1051/0004-6361/201015938},
  Eid                      = {A118},
  Eprint                   = {1012.0816},
  Keywords                 = {galaxies: spiral, galaxies: evolution, galaxies: ISM, galaxies: halos, galaxies: kinematics and dynamics},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Husemann2016,
  Title                    = {{The MUSE view of QSO PG 1307+085: an elliptical galaxy on the M$_{BH}$-{$\sigma$}$_{*}$ relation interacting with its group environment}},
  Author                   = {{Husemann}, B. and {Bennert}, V.~N. and {Scharw{\"a}chter}, J. and {Woo}, J.-H. and {Choudhury}, O.~S.},
  Journal                  = {\mnras},
  Year                     = {2016},

  Month                    = jan,
  Pages                    = {1905-1918},
  Volume                   = {455},

  Abstract                 = {We report deep optical integral-field spectroscopy with the Multi-Unit Spectroscopic Explorer (MUSE) at the Very Large Telescope of the luminous radio-quiet quasi-stellar object (QSO) PG 1307+085 obtained during commissioning. Given the high sensitivity and spatial resolution delivered by MUSE, we are able to resolve the compact (re ˜ 1.3 arcsec) elliptical host galaxy. After spectroscopic deblending of the QSO and host galaxy emission, we infer a stellar velocity dispersion of σ* = 155 ± 19 km s-1. This places PG 1307+085 on the local MBH-σ* relation within its intrinsic scatter but offset towards a higher black hole mass with respect to the mean relation. The MUSE observations reveal a large extended narrow-line region (ENLR) around PG 1307+085 reaching out to ˜30 kpc. In addition, we detect a faint ionized gas bridge towards the most massive galaxy of the galaxy group at 50 kpc distance. The ionized gas kinematics does not show any evidence for gas outflows on kpc scales despite the high QSO luminosity of Lbol > 1046 erg s-1. Based on the ionized gas distribution, kinematics and metallicity we discuss the origin of the ENLR with respect to its group environments including minor mergers, ram-pressure stripping or gas accretion as the likely scenarios. We conclude that PG 1307+085 is a normal elliptical host in terms of the scaling relations, but that the gas is likely affected by the environment through gravity or ambient pressure. It is possible that the interaction with the environment, seen in the ionized gas, might be responsible for driving sufficient gas to the black hole.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016MNRAS.455.1905H},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stv2478},
  Eprint                   = {1510.03864},
  Keywords                 = {techniques: imaging spectroscopy, ISM: abundances, galaxies: active, galaxies: bulges, galaxies: interactions, quasars: individual: PG 1307+085},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Jeans1922,
  Title                    = {{The motions of stars in a Kapteyn universe}},
  Author                   = {{Jeans}, J.~H.},
  Journal                  = {\mnras},
  Year                     = {1922},

  Month                    = jan,
  Pages                    = {122-132},
  Volume                   = {82},

  Abstract                 = {Not Available},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/1922MNRAS..82..122J},
  Comment                  = {Jeans},
  Doi                      = {10.1093/mnras/82.3.122},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Kormendy2013,
  Title                    = {Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies},
  Author                   = {Kormendy, John and Ho, Luis C.},
  Journal                  = {Annu. Rev. Astro. Astrophys.},
  Year                     = {2013},

  Month                    = {Aug},
  Number                   = {1},
  Pages                    = {511–653},
  Volume                   = {51},

  Comment                  = {Review},
  Doi                      = {10.1146/annurev-astro-082708-101811},
  File                     = {Published version:Kormendy2013.pdf:PDF},
  ISSN                     = {1545-4282},
  Owner                    = {sinead},
  Publisher                = {Annual Reviews},
  Timestamp                = {2015.12.11},
  Url                      = {http://dx.doi.org/10.1146/annurev-astro-082708-101811}
}

@Article{Krajnovic2009a,
  Title                    = {{Determination of masses of the central black holes in NGC 524 and 2549 using laser guide star adaptive optics}},
  Author                   = {{Krajnovi{\'c}}, D. and {McDermid}, R.~M. and {Cappellari}, M. and {Davies}, R.~L.},
  Journal                  = {\mnras},
  Year                     = {2009},

  Month                    = nov,
  Pages                    = {1839-1857},
  Volume                   = {399},

  Abstract                 = {We present observations of early-type galaxies NGC 524 and 2549 with laser guide star adaptive optics (LGS AO) obtained at GEMINI North telescope using the Near-infrared Integral Field Spectrograph (NIFS) integral field unit (IFU) in the K band. The purpose of these observations is to determine high spatial resolution stellar kinematics within the nuclei of these galaxies and, in combination with previously obtained large-scale observations with the SAURON IFU, to determine the masses (M•) of the supermassive black holes (SMBH). The targeted galaxies were chosen to have central light profiles showing a core (NGC 524) and a cusp (NGC 2549), to probe the feasibility of using the galaxy centre as the natural guide source required for LGS AO. We employ an innovative technique where the focus compensation due to the changing distance to the sodium layer is made `open loop', allowing the extended galaxy nucleus to be used only for tip-tilt correction. The data have spatial resolution of 0.23 and 0.17arcsec full-width at half maximum (FWHM), where at least ~40 per cent of flux comes within 0.2, showing that high quality LGS AO observations of these objects are possible. The achieved signal-to-noise ratio (S/N ~ 50) is sufficiently high to reliably determine the shape of the line-of-sight velocity distribution. We construct axisymmetric three-integral dynamical models which are constrained with both the NIFS and SAURON data. The best-fitting models yield M• = (8.3+2.7-1.3) × 108Msolar and (M/L)I = 5.8 +/- 0.4 for NGC 524 and M• = (1.4+0.2-1.3) × 107Msolar and (M/L)R = 4.7 +/- 0.2 for NGC 2549 (all errors are at the 3σ level). We demonstrate that the wide-field SAURON data play a crucial role in the M/L determination increasing the accuracy of M/L by a factor of at least 5, and constraining the upper limits on black hole masses. The NIFS data are crucial in constraining the lower limits of M• and in combination with the large-scale data reducing the uncertainty by a factor of 2 or more. We find that the orbital structure of NGC 524 shows significant tangential anisotropy, while at larger radii both galaxies are consistent with having almost perfectly oblate velocity ellipsoids. Tangential anisotropy in NGC 524 coincides with the size of SMBH sphere of influence and the core region in the light profile. This agrees with predictions from numerical simulations where core profiles are the result of SMBH binaries evacuating the centre nuclear regions following a galaxy merger. However, being a disc dominated fast rotating galaxy, NGC 524 has probably undergone through a more complex evolution. We test the accuracy to which M• can be measured using seeings obtained from typical LGS AO observations, and conclude that for a typical conditions and M• the expected uncertainty is of the order of 50 per cent.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009MNRAS.399.1839K},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1111/j.1365-2966.2009.15415.x},
  Eprint                   = {0907.3748},
  File                     = {Published version:Krajnovic2009a.pdf:PDF},
  Keywords                 = {NGC 524, NGC 2549},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Kuo2011,
  Title                    = {{The Megamaser Cosmology Project. III. Accurate Masses of Seven Supermassive Black Holes in Active Galaxies with Circumnuclear Megamaser Disks}},
  Author                   = {{Kuo}, C.~Y. and {Braatz}, J.~A. and {Condon}, J.~J. and {Impellizzeri}, C.~M.~V. and {Lo}, K.~Y. and {Zaw}, I. and {Schenker}, M. and {Henkel}, C. and {Reid}, M.~J. and {Greene}, J.~E.},
  Journal                  = {\apj},
  Year                     = {2011},

  Month                    = jan,
  Pages                    = {20},
  Volume                   = {727},

  Abstract                 = {Observations of H2O masers from circumnuclear disks in active galaxies for the Megamaser Cosmology Project (MCP) allow accurate measurement of the mass of supermassive black holes (BH) in these galaxies. We present the Very Long Baseline Interferometry images and kinematics of water maser emission in six active galaxies: NGC 1194, NGC 2273, NGC 2960 (Mrk 1419), NGC 4388, NGC 6264 and NGC 6323. We use the Keplerian rotation curves of these six megamaser galaxies, plus a seventh previously published, to determine accurate enclosed masses within the central ~0.3 pc of these galaxies, smaller than the radius of the sphere of influence of the central mass in all cases. We also set lower limits to the central mass densities of between 0.12 × 1010 and 61 × 1010 M sun pc-3. For six of the seven disks, the high central densities rule out clusters of stars or stellar remnants as the central objects, and this result further supports our assumption that the enclosed mass can be attributed predominantly to a supermassive BH. The seven BHs have masses ranging between 0.75 × 107 and 6.5 × 107 M sun, with the mass errors dominated by the uncertainty of the Hubble constant. We compare the megamaser BH mass determination with BH mass measured from the virial estimation method. The virial estimation BH mass in four galaxies is consistent with the megamaser BH mass, but the virial mass uncertainty is much greater. Circumnuclear megamaser disks allow the best mass determination of the central BH mass in external galaxies and significantly improve the observational basis at the low-mass end of the M-σsstarf relation. The M-σsstarf relation may not be a single, low-scatter power law as originally proposed. MCP observations continue and we expect to obtain more maser BH masses in the future.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011ApJ...727...20K},
  Archiveprefix            = {arXiv},
  Comment                  = {triaxial galaxies},
  Doi                      = {10.1088/0004-637X/727/1/20},
  Eid                      = {20},
  Eprint                   = {1008.2146},
  Keywords                 = {accretion, accretion disks, galaxies: active, galaxies: ISM, galaxies: nuclei, galaxies: Seyfert},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Lyubenova2008,
  Title                    = {{Central K-band kinematics and line strength maps of NGC 1399}},
  Author                   = {{Lyubenova}, M. and {Kuntschner}, H. and {Silva}, D.~R.},
  Journal                  = {\aap},
  Year                     = {2008},

  Month                    = jul,
  Pages                    = {425-433},
  Volume                   = {485},
  Abstract                 = {In this paper we present for the first time high spatial resolution K-band maps of the central kinematical and near-infrared spectral properties of the giant cD galaxy in the Fornax cluster, NGC 1399. We confirm the presence of a central velocity dispersion dip within r ≤ 0.2 arcsec seen in previous long-slit studies. Our velocity dispersion maps give evidence of a non-symmetric structure in this central area by showing three σ peaks to the north-east, south-east and west of the galaxy centre. Additionally we measure near-IR line strength indices at unprecedented spatial resolution in NGC 1399. The most important features we observe in our 2-dimensional line strength maps are drops in Na I and CO (2-0) line strength in the nuclear region of the galaxy, coinciding spatially with the drop in σ. The observed line strength and velocity dispersion changes suggest a scenario where the centre of NGC 1399 harbours a dynamically cold subsystem with a distinct stellar population.  Based on observation collected at the ESO Paranal La Silla Observatory, Chile, during the Science Verification of SINFONI.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008A%26A...485..425L},
  Archiveprefix            = {arXiv},
  Comment                  = {sigma-dip},
  Doi                      = {10.1051/0004-6361:20079314},
  Eprint                   = {0803.3806},
  File                     = {Published version:Lyubenova2008.pdf:PDF},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 1399, galaxies: kinematics and dynamics, galaxies: stellar content, galaxies: nuclei},
  Owner                    = {sinead},
  Timestamp                = {2016.02.18}
}

@Article{McDermid2015,
  Title                    = {{The ATLAS$^{3D}$ Project - XXX. Star formation histories and stellar population scaling relations of early-type galaxies}},
  Author                   = {{McDermid}, R.~M. and {Alatalo}, K. and {Blitz}, L. and {Bournaud}, F. and {Bureau}, M. and {Cappellari}, M. and {Crocker}, A.~F. and {Davies}, R.~L. and {Davis}, T.~A. and {de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Morganti}, R. and {Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and {Scott}, N. and {Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M. },
  Journal                  = {\mnras},
  Year                     = {2015},

  Month                    = apr,
  Pages                    = {3484-3513},
  Volume                   = {448},

  Abstract                 = {We present the stellar population content of early-type galaxies from the ATLAS3D survey. Using spectra integrated within apertures covering up to one effective radius, we apply two methods: one based on measuring line-strength indices and applying single stellar population (SSP) models to derive SSP-equivalent values of stellar age, metallicity, and alpha enhancement; and one based on spectral fitting to derive non-parametric star formation histories, mass-weighted average values of age, metallicity, and half-mass formation time-scales. Using homogeneously derived effective radii and dynamically determined galaxy masses, we present the distribution of stellar population parameters on the Mass Plane (MJAM, σe, R^maj_e), showing that at fixed mass, compact early-type galaxies are on average older, more metal-rich, and more alpha-enhanced than their larger counterparts. From non-parametric star formation histories, we find that the duration of star formation is systematically more extended in lower mass objects. Assuming that our sample represents most of the stellar content of today's local Universe, approximately 50 per cent of all stars formed within the first 2 Gyr following the big bang. Most of these stars reside today in the most massive galaxies (>1010.5 M⊙), which themselves formed 90 per cent of their stars by z ˜ 2. The lower mass objects, in contrast, have formed barely half their stars in this time interval. Stellar population properties are independent of environment over two orders of magnitude in local density, varying only with galaxy mass. In the highest density regions of our volume (dominated by the Virgo cluster), galaxies are older, alpha-enhanced, and have shorter star formation histories with respect to lower density regions.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015MNRAS.448.3484M},
  Archiveprefix            = {arXiv},
  Comment                  = {PPXF populations},
  Doi                      = {10.1093/mnras/stv105},
  Eprint                   = {1501.03723},
  Keywords                 = {galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: stellar content},
  Owner                    = {sinead},
  Timestamp                = {2015.12.15}
}

@Article{McDermid2006,
  Title                    = {{The SAURON project - VIII. OASIS/CFHT integral-field spectroscopy of elliptical and lenticular galaxy centres}},
  Author                   = {{McDermid}, R.~M. and {Emsellem}, E. and {Shapiro}, K.~L. and {Bacon}, R. and {Bureau}, M. and {Cappellari}, M. and {Davies}, R.~L. and {de Zeeuw}, T. and {Falc{\'o}n-Barroso}, J. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Peletier}, R.~F. and {Sarzi}, M.},
  Journal                  = {\mnras},
  Year                     = {2006},

  Month                    = dec,
  Pages                    = {906-958},
  Volume                   = {373},

  Abstract                 = {We present high spatial resolution integral-field spectroscopy of 28 elliptical (E) and lenticular (S0) galaxies from the SAURON representative survey obtained with the OASIS spectrograph during its operation at the Canada-France-Hawaii Telescope. These seeing-limited observations explore the central 8 × 10 arcsec2 (typically 1 kpc diameter) regions of these galaxies using a spatial sampling four times higher than SAURON (0.27-arcsec versus 0.94-arcsec spatial elements), resulting in almost a factor of 2 improvement in the median point spread function. These data allow accurate study of the central regions to complement the large-scale view provided by SAURON. Here we present the stellar and gas kinematics, stellar absorption-line strengths and nebular emission-line strengths for this sample. We also characterize the stellar velocity maps using the `kinemetry' technique, and derive maps of the luminosity-weighted stellar age, metallicity and abundance ratio via stellar population models. We give a brief review of the structures found in our maps, linking also to larger-scale structures measured with SAURON. We present two previously unreported kinematically decoupled components (KDCs) in the centres of NGC3032 and NGC4382. We compare the intrinsic size and luminosity-weighted stellar age of all the visible KDCs in the full SAURON sample, and find two types of components: kiloparsec-scale KDCs, which are older than 8 Gyr, and are found in galaxies with little net rotation; and compact KDCs, which have intrinsic diameters of less than a few hundred parsec, show a range of stellar ages from 0.5 to 15 Gyr (with 5/6 younger than 5 Gyr), are found exclusively in fast-rotating galaxies, and are close to counter-rotating around the same axis as their host. Of the seven galaxies in the SAURON sample with integrated luminosity-weighted ages less than 5 Gyr, five show such compact KDCs, suggesting a link between counter-rotation and recent star formation. We show that this may be due to a combination of small sample size at young ages, and an observational bias, since young KDCs are easier to detect than their older and/or corotating counterparts. Based on observations obtained at the Canada-France-Hawaii Telescope which is operated by the National Research Council of Canada, the Institut National des Sciences de l'Univers of the Centre National de la Recherche Scientifique of France, and the University of Hawaii. E-mail: mcdermid@strw.leidenuniv.nl},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2006MNRAS.373..906M},
  Comment                  = {PSF determination},
  Doi                      = {10.1111/j.1365-2966.2006.11065.x},
  Eprint                   = {astro-ph/0609452},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: structure},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{McDermid2006a,
  Title                    = {{The SAURON project - VIII. OASIS/CFHT integral-field spectroscopy of elliptical and lenticular galaxy centres}},
  Author                   = {{McDermid}, R.~M. and {Emsellem}, E. and {Shapiro}, K.~L. and {Bacon}, R. and {Bureau}, M. and {Cappellari}, M. and {Davies}, R.~L. and {de Zeeuw}, T. and {Falc{\'o}n-Barroso}, J. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and {Peletier}, R.~F. and {Sarzi}, M.},
  Journal                  = {\mnras},
  Year                     = {2006},

  Month                    = dec,
  Pages                    = {906-958},
  Volume                   = {373},
  Abstract                 = {We present high spatial resolution integral-field spectroscopy of 28 elliptical (E) and lenticular (S0) galaxies from the SAURON representative survey obtained with the OASIS spectrograph during its operation at the Canada-France-Hawaii Telescope. These seeing-limited observations explore the central 8 × 10 arcsec2 (typically 1 kpc diameter) regions of these galaxies using a spatial sampling four times higher than SAURON (0.27-arcsec versus 0.94-arcsec spatial elements), resulting in almost a factor of 2 improvement in the median point spread function. These data allow accurate study of the central regions to complement the large-scale view provided by SAURON. Here we present the stellar and gas kinematics, stellar absorption-line strengths and nebular emission-line strengths for this sample. We also characterize the stellar velocity maps using the `kinemetry' technique, and derive maps of the luminosity-weighted stellar age, metallicity and abundance ratio via stellar population models. We give a brief review of the structures found in our maps, linking also to larger-scale structures measured with SAURON. We present two previously unreported kinematically decoupled components (KDCs) in the centres of NGC3032 and NGC4382. We compare the intrinsic size and luminosity-weighted stellar age of all the visible KDCs in the full SAURON sample, and find two types of components: kiloparsec-scale KDCs, which are older than 8 Gyr, and are found in galaxies with little net rotation; and compact KDCs, which have intrinsic diameters of less than a few hundred parsec, show a range of stellar ages from 0.5 to 15 Gyr (with 5/6 younger than 5 Gyr), are found exclusively in fast-rotating galaxies, and are close to counter-rotating around the same axis as their host. Of the seven galaxies in the SAURON sample with integrated luminosity-weighted ages less than 5 Gyr, five show such compact KDCs, suggesting a link between counter-rotation and recent star formation. We show that this may be due to a combination of small sample size at young ages, and an observational bias, since young KDCs are easier to detect than their older and/or corotating counterparts.  Based on observations obtained at the Canada-France-Hawaii Telescope which is operated by the National Research Council of Canada, the Institut National des Sciences de l'Univers of the Centre National de la Recherche Scientifique of France, and the University of Hawaii.  E-mail: mcdermid@strw.leidenuniv.nl},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2006MNRAS.373..906M},
  Comment                  = {PSF},
  Doi                      = {10.1111/j.1365-2966.2006.11065.x},
  Eprint                   = {astro-ph/0609452},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: structure},
  Owner                    = {sinead},
  Timestamp                = {2016.02.18}
}

@Article{Nowak2008,
  Title                    = {{The supermassive black hole of FornaxA}},
  Author                   = {{Nowak}, N. and {Saglia}, R.~P. and {Thomas}, J. and {Bender}, R. and {Davies}, R.~I. and {Gebhardt}, K.},
  Journal                  = {\mnras},
  Year                     = {2008},

  Month                    = dec,
  Pages                    = {1629-1649},
  Volume                   = {391},

  Abstract                 = {The radio galaxy FornaxA (NGC 1316) is a prominent merger remnant in the outskirts of the Fornax cluster. Its giant radio lobes suggest the presence of a powerful active galactic nuclei (AGN) and thus a central supermassive black hole (SMBH). FornaxA now seems to be in a transition state between active black hole growth and quiescence, as indicated by the strongly declined activity of the nucleus. Studying objects in this evolutionary phase is particularly important in order to understand the link between bulge formation and black hole growth, which is manifested in the M•-σ relation between black hole mass and bulge velocity dispersion. So far, a measurement of the SMBH mass has not been possible in FornaxA, as it is enshrouded in dust which makes optical measurements impossible. We present high-resolution adaptive optics assisted integral-field data of FornaxA, taken with SINFONI at the Very Large Telescope in the K band, where the influence of dust is negligible. The achieved spatial resolution is 0.085 arcsec, which is about a fifth of the diameter of the expected sphere of influence of the black hole. The stellar kinematics was measured using the region around the CO bandheads at 2.3 μm. FornaxA does not rotate inside the inner ~3 arcsec. The velocity dispersion increases towards the centre. The weak AGN emission affects the stellar kinematics in the inner ~0.06 arcsec only. Beyond this radius, the stellar kinematics appears relaxed in the central regions. We use axisymmetric orbit models to determine the mass of the SMBH in the centre of FornaxA. The three-dimensional nature of our data provides the possibility to directly test the consistency of the data with axisymmetry by modelling each of the four quadrants separately. According to our dynamical models, consistent SMBH masses M• and dynamical Ks-band mass-to-light ratios Υ are obtained for all quadrants, with <M•> = 1.3 × 108Msolar [rms(M•) = 0.4 × 108Msolar] and <Υ> = 0.68 [rms(Υ) = 0.03], confirming the assumption of axisymmetry. For the folded and averaged data, we find M• = 1.5+0.75-0.8 × 108Msolar and Υ = 0.65+0.075-0.05 (3σ errors). Thus, the black hole mass of FornaxA is consistent within the error with the Tremaine et al. M•-σ relation, but is a factor of ~4 smaller than expected from its bulge mass and the Marconi & Hunt relation. Based on observations at the European Southern Observatory (ESO) Very Large Telescope [076.B-0457(A)] and archival ESO La Silla [66.C-0310(A)] and NASA/ESA Hubble Space Telescope data (GO Proposal 7458), obtained from the ESO/ST-ECF Science Archive Facility. E-mail: nnowak@mpe.mpg.de},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008MNRAS.391.1629N},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1111/j.1365-2966.2008.13960.x},
  Eprint                   = {0809.0696},
  File                     = {Published version:Nowak2008.pdf:PDF},
  Keywords                 = {galaxies: individual: NGC 1316 (Fornax A) , galaxies: kinematics and dynamics},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Oka2016,
  Title                    = {{Signature of an Intermediate-mass Black Hole in the Central Molecular Zone of Our Galaxy}},
  Author                   = {{Oka}, T. and {Mizuno}, R. and {Miura}, K. and {Takekawa}, S. },
  Journal                  = {\apjl},
  Year                     = {2016},

  Month                    = jan,
  Pages                    = {L7},
  Volume                   = {816},
  Abstract                 = {We mapped the high-velocity compact cloud CO-0.40-0.22 in 21 molecular lines in the 3 mm band using the Nobeyama Radio Observatory 45 m radio telescope. Eighteen lines were detected from CO-0.40-0.22. The map of each detected line shows that this cloud has a compact appearance (d ≃ 3 pc) and extremely broad velocity width (ΔV ≃ 100 km s-1). The mass and kinetic energy of CO-0.40-0.22 are estimated to be 103.6 M⊙ and 1049.7 erg, respectively. The representative position-velocity map along the major axis shows that CO-0.40-0.22 consists of an intense region with a shallow velocity gradient and a less intense high-velocity wing. Here, we show that this kinematical structure can be attributed to a gravitational kick to the molecular cloud caused by an invisible compact object with a mass of ˜105 M⊙. Its compactness and the absence of counterparts at other wavelengths suggest that this massive object is an intermediate-mass black hole.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016ApJ...816L...7O},
  Archiveprefix            = {arXiv},
  Doi                      = {10.3847/2041-8205/816/1/L7},
  Eid                      = {L7},
  Eprint                   = {1512.04661},
  Keywords                 = {galaxies: nuclei, Galaxy: center, ISM: clouds, ISM: molecules},
  Owner                    = {sinead},
  Timestamp                = {2016.01.18}
}

@Article{Qian1995,
  Title                    = {{Axisymmetric galaxy models with central black holes, with an application to M32}},
  Author                   = {{Qian}, E.~E. and {de Zeeuw}, P.~T. and {van der Marel}, R.~P. and {Hunter}, C.},
  Journal                  = {\mnras},
  Year                     = {1995},

  Month                    = may,
  Pages                    = {602-622},
  Volume                   = {274},

  Abstract                 = {The contour integral method of Hunter & Qian is applied to axisymmetric galaxy models in which the distribution function (DF) is of the form f=f(E, L_z), where E and L_z are the classical integrals of motion in an axisymmetric potential. A practical way to construct the unique even part fe(E, L_z) of the two-integral DF for such systems is presented. It is applied to models, both oblate and prolate, in which the mass density is stratified on similar concentric spheroids. The spheroids with scale-free densities are discussed in detail. These provide useful approximations to the behaviour of more realistic models in the limit of small and large radii. The self-consistent case is treated, as well as the case in which there are additional contributions to the potential from a central black hole or dark halo. The two-integral DFs for scale-free densities in a Kepler potential are particularly simple. These can be used to model power-law density cusps near a central black hole, or to model the outer parts of finite-mass systems. The range of axial ratios and density profile slopes is determined for which spheroidal power-law cusps with a central black hole have a physical two-integral DF. More generally, the two-integral DFs are discussed for a set of spheroidal `(alpha,beta)-models', characterized by a power-law density cusp with slope alpha at small radii, and a power-law density fall-off with slope alpha + 2 beta at large radii. As an application, the DF is constructed for the (alpha,beta)-model with a 1.8 x 10^6 M_solar black hole used by van der Marel et al.to interpret their high spatial resolution spectroscopic data for M32. The line-of-sight velocity profiles are calculated. The results confirm that the model fits the data remarkably well. The model is used to calculate the predicted kinematic signatures of a central black hole in M32 in spectroscopic observations through small apertures, such as are now possible with the Faint Object Spectrograph on board the Hubble Space Telescope.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/1995MNRAS.274..602Q},
  Comment                  = {Kernel - velocity convolution},
  Doi                      = {10.1093/mnras/274.2.602},
  Eprint                   = {astro-ph/9412067},
  Keywords                 = {BLACK HOLE PHYSICS, CELESTIAL MECHANICS, STELLAR DYNAMICS, GALAXIES: INDIVIDUAL: M32, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: STRUCTURE},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Reines2015,
  Title                    = {{Relations between Central Black Hole Mass and Total Galaxy Stellar Mass in the Local Universe}},
  Author                   = {{Reines}, A.~E. and {Volonteri}, M.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = nov,
  Pages                    = {82},
  Volume                   = {813},

  Abstract                 = {Scaling relations between central black hole (BH) mass and host galaxy properties are of fundamental importance to studies of BH and galaxy evolution throughout cosmic time. Here we investigate the relationship between BH mass and host galaxy total stellar mass using a sample of 262 broad-line active galactic nuclei (AGNs) in the nearby universe (z < 0.055), as well as 79 galaxies with dynamical BH masses. The vast majority of our AGN sample is constructed using Sloan Digital Sky Survey spectroscopy and searching for Seyfert-like narrow-line ratios and broad Hα emission. BH masses are estimated using standard virial techniques. We also include a small number of dwarf galaxies with total stellar masses Mstellar ≲ 109.5 M⊙ and a subsample of the reverberation-mapped AGNs. Total stellar masses of all 341 galaxies are calculated in the most consistent manner feasible using color-dependent mass-to-light ratios. We find a clear correlation between BH mass and total stellar mass for the AGN host galaxies, with MBH ∝ Mstellar, similar to that of early-type galaxies with dynamically detected BHs. However, the relation defined by the AGNs has a normalization that is lower by more than an order of magnitude, with a BH-to-total stellar mass fraction of MBH/Mstellar ∼ 0.025% across the stellar mass range 108 ≤ Mstellar/M⊙ ≤ 1012. This result has significant implications for studies at high redshift and cosmological simulations in which stellar bulges cannot be resolved.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...813...82R},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/813/2/82},
  Eid                      = {82},
  Eprint                   = {1508.06274},
  Keywords                 = {galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: Seyfert},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Rusli2013,
  Title                    = {{The Influence of Dark Matter Halos on Dynamical Estimates of Black Hole Mass: 10 New Measurements for High-{$\sigma$} Early-type Galaxies}},
  Author                   = {{Rusli}, S.~P. and {Thomas}, J. and {Saglia}, R.~P. and {Fabricius}, M. and {Erwin}, P. and {Bender}, R. and {Nowak}, N. and {Lee}, C.~H. and {Riffeser}, A. and {Sharp}, R.},
  Journal                  = {\aj},
  Year                     = {2013},

  Month                    = sep,
  Pages                    = {45},
  Volume                   = {146},

  Abstract                 = {Adaptive optics assisted SINFONI observations of the central regions of 10 early-type galaxies are presented. Based primarily on the SINFONI kinematics, 10 black hole (BH) masses occupying the high-mass regime of the M BH-σ relation are derived using three-integral Schwarzschild models. The effect of dark matter (DM) inclusion on the BH mass is explored. The omission of a DM halo in the model results in a higher stellar mass-to-light ratio, especially when extensive kinematic data are used in the model. However, when the diameter of the sphere of influence—computed using the BH mass derived without a dark halo—is at least 10 times the point-spread function FWHM during the observations, it is safe to exclude a DM component in the dynamical modeling, i.e., the change in BH mass is negligible. When the spatial resolution is marginal, restricting the mass-to-light ratio to the right value returns the correct M BH although a dark halo is not present in the model. Compared to the M BH-σ and M BH-L relations of McConnell et al., the 10 BHs are all more massive than expected from the luminosities and 7 BH masses are higher than expected from the stellar velocity dispersions of the host bulges. Using new fitted relations, which include the 10 galaxies, we find that the space density of the most massive BHs (M BH >~ 109 M ⊙) estimated from the M BH-L relation is higher than the estimate based on the M BH-σ relation and the latter is higher than model predictions based on quasar counts, each by about an order of magnitude. Based on observations at the European Southern Observatory Very Large Telescope (082.B-0037(A), 083.B-0126(A), 082.B-0037(B), and 086.B-0085(A)). This paper includes data taken at The McDonald Observatory of The University of Texas at Austin.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2013AJ....146...45R},
  Archiveprefix            = {arXiv},
  Comment                  = {BH talk 2014},
  Doi                      = {10.1088/0004-6256/146/3/45},
  Eid                      = {45},
  Eprint                   = {1306.1124},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: nuclei},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Sanchez-Blazquez2006,
  Title                    = {{Medium-resolution Isaac Newton Telescope library of empirical spectra}},
  Author                   = {{S{\'a}nchez-Bl{\'a}zquez}, P. and {Peletier}, R.~F. and {Jim{\'e}nez-Vicente}, J. and {Cardiel}, N. and {Cenarro}, A.~J. and {Falc{\'o}n-Barroso}, J. and {Gorgas}, J. and {Selam}, S. and {Vazdekis}, A.},
  Journal                  = {\mnras},
  Year                     = {2006},

  Month                    = sep,
  Pages                    = {703-718},
  Volume                   = {371},

  __markedentry            = {[sinead:]},
  Abstract                 = {A new stellar library developed for stellar population synthesis modelling is presented. The library consists of 985 stars spanning a large range in atmospheric parameters. The spectra were obtained at the 2.5-m Isaac Newton Telescope and cover the range λλ 3525-7500 Å at 2.3 Å (full width at half-maximum) spectral resolution. The spectral resolution, spectral-type coverage, flux-calibration accuracy and number of stars represent a substantial improvement over previous libraries used in population-synthesis models.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2006MNRAS.371..703S},
  Comment                  = {MILES},
  Doi                      = {10.1111/j.1365-2966.2006.10699.x},
  Eprint                   = {astro-ph/0607009},
  Keywords                 = {atlases: stars: fundamental parameters: galaxies: stellar content, atlases, stars: fundamental parameters, galaxies: stellar content},
  Owner                    = {sinead},
  Timestamp                = {2016.02.18}
}

@Article{Satyapal2008,
  Title                    = {{Spitzer Uncovers Active Galactic Nuclei Missed by Optical Surveys in Seven Late-Type Galaxies}},
  Author                   = {{Satyapal}, S. and {Vega}, D. and {Dudik}, R.~P. and {Abel}, N.~P. and {Heckman}, T.},
  Journal                  = {\apj},
  Year                     = {2008},

  Month                    = apr,
  Pages                    = {926-942},
  Volume                   = {677},

  Abstract                 = {We report the discovery using Spitzer's high-resolution spectrograph of seven active galactic nuclei (AGNs) in a sample of 32 late-type galaxies that show no definitive signatures of AGNs in their optical spectra. These observations suggest that the AGN detection rate in late-type galaxies is possibly 4 times larger than what optical spectroscopic observations alone suggest. We demonstrate using photoionization models with an input AGN and an extreme UV-bright starburst ionizing radiation field that the observed mid-infrared line spectrum, which includes the high-ionization [Ne V] 14 μm and/or 24 μm lines, cannot be replicated unless an AGN contribution, in some cases as little as 10% of the total galaxy luminosity, is included. These models show that when the fraction of the total luminosity due to the AGN is low, optical diagnostics are insensitive to the presence of the AGN. In this regime of parameter space, the mid-infrared diagnostics offer a powerful tool for uncovering AGNs missed by optical spectroscopy. The AGN bolometric luminosities in our sample range from ~3×1041 to ~2×1043 ergs s-1, which, based on the Eddington limit, corresponds to a lower mass limit for the black hole that ranges from ~3×103 to as high as ~1.5×105 Msolar. These lower mass limits, however, do not put a strain on the well-known relationship between the black hole mass and the host galaxy's stellar velocity dispersion established in predominantly early-type galaxies. Our findings add to the growing evidence that black holes do form and grow in low-bulge environments and that they are significantly more common than optical studies indicate.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008ApJ...677..926S},
  Archiveprefix            = {arXiv},
  Comment                  = {no AGN, no central star formation},
  Doi                      = {10.1086/529014},
  Eprint                   = {0801.2759},
  Keywords                 = {Black Hole Physics, Cosmology: Dark Matter, Galaxies: Active, Galaxies: Spiral, Infrared: Galaxies},
  Owner                    = {sinead},
  Timestamp                = {2015.12.18}
}

@Article{Schulze2011,
  Title                    = {{Selection effects in the black hole-bulge relation and its evolution}},
  Author                   = {{Schulze}, A. and {Wisotzki}, L.},
  Journal                  = {\aap},
  Year                     = {2011},

  Month                    = nov,
  Pages                    = {A87},
  Volume                   = {535},

  Abstract                 = {We present an investigation of sample selection effects that influence the observed black hole-bulge relations and its evolution with redshift. We provide a common framework in which all kinds of selection effects on the M•-bulge relations can be investigated, but our main emphasis is on the consequences of using broad-line AGN with virial estimates of black hole masses and their host galaxies to search for evolution in the BH-bulge relation. We identified relevant sources of bias that were not discussed in the literature so far. A particularly important effect is caused by the fact that the active fraction among SMBHs varies considerably with BH mass, in the sense that high-mass BHs are less likely to be active than lower mass ones. In the connection with intrinsic scatter of the BH-bulge relation this effect implies a bias towards a low BH mass at given bulge property. This effect adds to the bias caused by working with luminosity or flux limited samples that were already discussed by others. A quantitative prediction of these biases requires (i) a realistic model of the sample selection function, and (ii) knowledge of relevant underlying distribution functions: the distribution of spheroid properties such as velocity dispersions or masses; the active fraction as a function of BH mass, or alternatively the active black hole mass function; and the Eddington ratio distribution function. We employed our formalism together with recently determined distribution functions to investigate how much existing studies of the M•-bulge relation using AGN hosts might suffer from selection biases. For low-redshift AGN samples we can naturally reproduce the flattening of the relation observed in some studies without having to invoke intrinsic differences in the BH-bulge relation between active and inactive galaxies. When extending our analysis to higher redshift samples we are clearly hampered by limited empirical constraints on the various relevant distribution functions. Using a best-guess approach for these distributions we estimate the expected magnitude of sample selection biases for a number of recent observational attempts to study the M•-bulge evolution. In no case do we find statistically significant evidence for an evolving M•-bulge relation. While the observed apparent offsets in M• /MBulge from the local relation can be quite large, the sample selection bias estimated from our formalism is typically of the same magnitude. We suggest a possible practical approach to circumvent several of the most problematic issues connected with AGN selection; this could become a powerful diagnostic in future investigations.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2011A%26A...535A..87S},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361/201117564},
  Eid                      = {A87},
  Eprint                   = {1109.2787},
  Keywords                 = {galaxies: active, galaxies: nuclei, quasars: general},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Scott2009,
  Title                    = {{The SAURON Project - XIV. No escape from V$_{esc}$: a global and local parameter in early-type galaxy evolution}},
  Author                   = {{Scott}, N. and {Cappellari}, M. and {Davies}, R.~L. and {Bacon}, R. and {de Zeeuw}, P.~T. and {Emsellem}, E. and {Falc{\'o}n-Barroso}, J. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and {McDermid}, R.~M. and {Peletier}, R.~F. and {Pipino}, A. and {Sarzi}, M. and {van den Bosch}, R.~C.~E. and {van de Ven}, G. and {van Scherpenzeel}, E.},
  Journal                  = {\mnras},
  Year                     = {2009},

  Month                    = oct,
  Pages                    = {1835-1857},
  Volume                   = {398},

  Abstract                 = {We present the results of an investigation of the local escape velocity (Vesc) - line strength index relationship for 48 early-type galaxies from the SAURON sample, the first such study based on a large sample of galaxies with both detailed integral field observations and extensive dynamical modelling. Values of Vesc are computed using multi-Gaussian expansion (MGE) photometric fitting and axisymmetric, anisotropic Jeans' dynamical modelling simultaneously on Hubble Space Telescope and ground-based images. We determine line strengths and escape velocities at multiple radii within each galaxy, allowing an investigation of the correlation within individual galaxies as well as amongst galaxies. We find a tight correlation between Vesc and the line-strength indices. For Mgb, we find that this correlation exists not only between different galaxies but also inside individual galaxies - it is both a local and global correlation. The Mgb-Vesc relation has the form: log(Mgb/4Å) = (0.32 +/- 0.03) log(Vesc/500km s-1) - (0.031 +/- 0.007) with an rms scatter σ = 0.033. The relation within individual galaxies has the same slope and offset as the global relation to a good level of agreement, though there is significant intrinsic scatter in the local gradients. We transform our line strength index measurements to the single stellar population (SSP) equivalent ages (t), metallicity ([Z/H]) and enhancement ([α/Fe]) and carry out a principal component analysis of our SSP and Vesc data. We find that in this four-dimensional parameter space the galaxies in our sample are to a good approximation confined to a plane, given by log (V esc/500 kms -1) = 0.85 [Z/H] + 0.43 log (t/Gyr) - 0.29. It is surprising that a combination of age and metallicity is conserved; this may indicate a `conspiracy' between age and metallicity or a weakness in the SSP models. How the connection between stellar populations and the gravitational potential, both locally and globally, is preserved as galaxies assemble hierarchically may provide an important constraint on modelling.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009MNRAS.398.1835S},
  Archiveprefix            = {arXiv},
  Comment                  = {JAM},
  Doi                      = {10.1111/j.1365-2966.2009.15275.x},
  Eprint                   = {0906.3321},
  File                     = {arXiv v1:Scott2009-eprintv1.pdf:PDF},
  Keywords                 = {galaxies: abundances , galaxies: elliptical and lenticular, cD , galaxies: evolution , galaxies: formation},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.GA},
  Timestamp                = {2015.12.18}
}

@Article{Scott2013,
  Title                    = {{The ATLAS$^{3D}$ project - XXI. Correlations between gradients of local escape velocity and stellar populations in early-type galaxies}},
  Author                   = {{Scott}, N. and {Cappellari}, M. and {Davies}, R.~L. and {Kleijn}, G.~V. and {Bois}, M. and {Alatalo}, K. and {Blitz}, L. and {Bournaud}, F. and {Bureau}, M. and {Crocker}, A. and {Davis}, T.~A. and {de Zeeuw}, P.~T. and {Duc}, P.-A. and {Emsellem}, E. and {Khochfar}, S. and {Krajnovi{\'c}}, D. and {Kuntschner}, H. and {McDermid}, R.~M. and {Morganti}, R. and {Naab}, T. and {Oosterloo}, T. and {Sarzi}, M. and {Serra}, P. and {Weijmans}, A.-M. and {Young}, L.~M.},
  Journal                  = {\mnras},
  Year                     = {2013},

  Month                    = jul,
  Pages                    = {1894-1913},
  Volume                   = {432},

  Abstract                 = {We explore the connection between the local escape velocity, Vesc, and the stellar population properties in the ATLAS3D survey, a complete, volume-limited sample of nearby early-type galaxies. We make use of ugriz photometry to construct Multi-Gaussian Expansion models of the surface brightnesses of our galaxies. We are able to fit the full range of surface brightness profiles found in our sample, and in addition we reproduce the results of state-of-the-art photometry in the literature with residuals of 0.04 mag. We utilize these photometric models and SAURON integral-field spectroscopy, combined with Jeans dynamical modelling, to determine the local Vesc derived from the surface brightness. We find that the local Vesc is tightly correlated with the Mg b and Fe5015 line strengths and optical colours, and anti-correlated with the Hβ line strength. In the case of the Mg b and colour-Vesc relations we find that the relation within individual galaxies follows the global relation between different galaxies. We intentionally ignored any uncertain contribution due to dark matter since we are seeking an empirical description of stellar population gradients in early-type galaxies that is ideal for quantitative comparison with model predictions. We also make use of single stellar population (SSP) modelling to transform our line strength index measurements into the SSP-equivalent parameters age (t), metallicity ([Z/H]) and α-enhancement [α/Fe]. The residuals from the relation are correlated with age, [α/Fe], molecular gas mass and local environmental density. We identify a population of galaxies that occur only at low Vesc that exhibit negative gradients in the Mg b- and Colour-Vesc relations. These galaxies typically have young central stellar populations and contain significant amounts of molecular gas and dust. Combining these results with N-body simulations of binary mergers we use the Mg b-Vesc relation to constrain the possible number of dry mergers experienced by the local early-type galaxy population - a typical massive early-type galaxy can have experienced only ˜1.5 major mergers before becoming a significant outlier in the Mg b-Vesc relation.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2013MNRAS.432.1894S},
  Archiveprefix            = {arXiv},
  Comment                  = {dust correction},
  Doi                      = {10.1093/mnras/sts422},
  Eprint                   = {1211.4615},
  Keywords                 = {galaxies: abundances, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Seth2014,
  Title                    = {{A supermassive black hole in an ultra-compact dwarf galaxy}},
  Author                   = {{Seth}, A.~C. and {van den Bosch}, R. and {Mieske}, S. and {Baumgardt}, H. and {Brok}, M.~D. and {Strader}, J. and {Neumayer}, N. and {Chilingarian}, I. and {Hilker}, M. and {McDermid}, R. and {Spitler}, L. and {Brodie}, J. and {Frank}, M.~J. and {Walsh}, J.~L.},
  Journal                  = {\nat},
  Year                     = {2014},

  Month                    = sep,
  Pages                    = {398-400},
  Volume                   = {513},

  Abstract                 = {Ultra-compact dwarf galaxies are among the densest stellar systems in the Universe. These systems have masses of up to 2 × 108 solar masses, but half-light radii of just 3-50 parsecs. Dynamical mass estimates show that many such dwarfs are more massive than expected from their luminosity. It remains unclear whether these high dynamical mass estimates arise because of the presence of supermassive black holes or result from a non-standard stellar initial mass function that causes the average stellar mass to be higher than expected. Here we report adaptive optics kinematic data of the ultra-compact dwarf galaxy M60-UCD1 that show a central velocity dispersion peak exceeding 100 kilometres per second and modest rotation. Dynamical modelling of these data reveals the presence of a supermassive black hole with a mass of 2.1 × 107 solar masses. This is 15 per cent of the object's total mass. The high black hole mass and mass fraction suggest that M60-UCD1 is the stripped nucleus of a galaxy. Our analysis also shows that M60-UCD1's stellar mass is consistent with its luminosity, implying a large population of previously unrecognized supermassive black holes in other ultra-compact dwarf galaxies.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2014Natur.513..398S},
  Archiveprefix            = {arXiv},
  Comment                  = {dwarf galaxy},
  Doi                      = {10.1038/nature13762},
  Eprint                   = {1409.4769},
  File                     = {arXiv v2:Seth2014-eprintv2.pdf:PDF},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Shetty2015,
  Title                    = {{Observed trend in the star formation history and the dark matter fraction of galaxies at redshift z {\ap} 0.8}},
  Author                   = {{Shetty}, S. and {Cappellari}, M.},
  Journal                  = {\mnras},
  Year                     = {2015},

  Month                    = dec,
  Pages                    = {1332-1357},
  Volume                   = {454},

  Abstract                 = {We study the star formation history for a sample of 154 galaxies with stellar mass 10^{10}≲ M_{*} ≲ 10^{12} { M_{⊙}} in the redshift range 0.7 < z < 0.9. We do this using stellar population models combined with full-spectrum fitting of good quality spectra and high-resolution photometry. For a subset of 68 galaxies (M_{*}≳ 10^{11}{ M_{⊙}}) we additionally construct dynamical models. These use an axisymmetric solution to the Jeans equations, which allows for velocity anisotropy, and adopts results from abundance matching techniques to account for the dark matter content. We find that (i) the trends in star formation history observed in the local Universe are already in place by z ˜ 1: the most massive galaxies are already passive, while lower mass ones have a more extended star formation histories, and the lowest mass galaxies are actively forming stars; (ii) we place an upper limit of a factor 1.5 to the size growth of the massive galaxy population; (iii) we present strong evidence for low dark matter fractions within 1Re (median of 9 per cent and 90th percentile of 21 per cent) for galaxies with M_{*} ≳ 10^{11} { M_{⊙}} at these redshifts; and (iv) we confirm that these galaxies have, on average, a Salpeter normalization of the stellar initial mass function.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015MNRAS.454.1332S},
  Archiveprefix            = {arXiv},
  Comment                  = {PPXF population determination, determine M/L},
  Doi                      = {10.1093/mnras/stv1948},
  Eprint                   = {1508.05009},
  Keywords                 = {galaxies: evolution, galaxies: formation, galaxies: haloes, galaxies: high redshift, galaxies: star formation, galaxies: stellar content},
  Owner                    = {sinead},
  Timestamp                = {2015.12.15}
}

@Article{Vallejo2002,
  Title                    = {{The stellar mass to light ratio in the isolated spiral NGC 4414}},
  Author                   = {{Vallejo}, O. and {Braine}, J. and {Baudry}, A.},
  Journal                  = {\aap},
  Year                     = {2002},

  Month                    = may,
  Pages                    = {429-440},
  Volume                   = {387},

  Abstract                 = {We present high resolution CO(1-0) interferometric observations and deep HST B-V-I images of the flocculent isolated Sc type spiral NGC 4414. The goal is to determine the stellar mass-to-light (M/L) ratio in a galactic disk. NGC 4414 is an ideal object for this kind of study, as it is an unperturbed object at high galactic latitude with very extended atomic gas (HI). Many Cepheid light curves were measured in NGC 4414 so its distance is known to be about 19.2 Mpc. NGC 4414 is quite axisymmetric, with no bar and poorly defined spiral structure, and the center is seen unobscured (no CO, HI, Hα , or thermal dust emission near the nucleus), as in many isolated spiral galaxies. Not only does this result in minimal non-circular velocities but also, and this is a key to our success, the central light profile traces the total mass. The stars are seen without a dust screen, the central gas mass is very low (undetected), and we show that the dark matter is negligible in the central regions. We have developed an axisymmetric analytical gravitational potential model to account for the central light (mass) profile, the dynamics of the molecular gas in the highly obscured molecular ring, and the stellar light profile outside the highly obscured region. A single dominant disk component reproduces the disk dynamics and outer stellar light profile such that even if other disk components were present they would not affect our results. The contribution of dark matter is constrained by the extremely extended HI rotation curve and is small, possibly negligible, at distances less than 5-7 kpc from the center. Furthermore, the M/L ratios we derive are low, about 1.5 in I band and 0.5 in K' band. The B and V band M/L ratios vary greatly due to absorption by dust, reaching 4 in the molecular ring and decreasing to about 1.6-1.8 at larger radii. This unequivocally shows that models, like most maximum disk models, assuming constant M/L ratios in an optical waveband, simply are not appropriate. We illustrate this by making mock maximum disk models with a constant V band M/L ratio. The key is having the central light distribution unobscured such that it can be used to trace the mass. The K' band M/L ratio is virtually constant over the disk, suggesting that the intrinsic (unobscured) stellar M/L ratio is roughly constant. A primitive attempt to determine the intrinsic M/L ratio yields values close to unity in the B, V, and I bands and slightly below 0.5 in K'.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2002A%26A...387..429V},
  Comment                  = {M/L},
  Doi                      = {10.1051/0004-6361:20020261},
  Eprint                   = {astro-ph/0202391},
  File                     = {Published version:Vallejo2002.pdf:PDF},
  Keywords                 = {NGC 4414},
  Owner                    = {sinead},
  Timestamp                = {2015.12.15}
}

@Article{vandenBosch2010,
  Title                    = {{Estimating black hole masses in triaxial galaxies}},
  Author                   = {{van den Bosch}, R.~C.~E. and {de Zeeuw}, P.~T.},
  Journal                  = {\mnras},
  Year                     = {2010},

  Month                    = jan,
  Pages                    = {1770-1780},
  Volume                   = {401},

  Abstract                 = {Most of the supermassive black hole mass (M•) estimates based on stellar kinematics use the assumption that galaxies are axisymmetric oblate spheroids or spherical. Here, we use fully general triaxial orbit-based models to explore the effect of relaxing the axisymmetric assumption on the previously studied galaxies M32 and NGC 3379. We find that M32 can only be modelled accurately using an axisymmetric shape viewed nearly edge-on, and our black hole mass estimate is identical to previous studies. When the observed 5° kinematical twist is included in our model of NGC 3379, the best shape is mildly triaxial, and we find that our best-fitting black hole mass estimate doubles with respect to the axisymmetric model. This particular black hole mass estimate is still within the errors of that of the axisymmetric model and consistent with the M•-σ relationship. However, this effect may have a pronounced impact on black hole demography, since roughly a third of the most massive galaxies are strongly triaxial.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2010MNRAS.401.1770V},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1111/j.1365-2966.2009.15832.x},
  Eprint                   = {0910.0844},
  Keywords                 = {black hole physics, galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 3379, galaxies: individual: M32, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.CO},
  Timestamp                = {2015.12.21}
}

@Article{Walsh2010,
  Title                    = {{The Supermassive Black Hole in M84 Revisited}},
  Author                   = {{Walsh}, J.~L. and {Barth}, A.~J. and {Sarzi}, M.},
  Journal                  = {\apj},
  Year                     = {2010},

  Month                    = sep,
  Pages                    = {762-776},
  Volume                   = {721},

  Abstract                 = {The mass of the central black hole in the giant elliptical galaxy M84 has previously been measured by two groups using the same observations of emission-line gas with the Space Telescope Imaging Spectrograph (STIS) on the Hubble Space Telescope, giving strongly discrepant results: Bower et al. found M BH = (1.5+1.1 -0.6) × 109 M sun, while Maciejewski & Binney estimated M BH = 4 × 108 M sun. In order to resolve this discrepancy, we have performed new measurements of the gas kinematics in M84 from the same archival data and carried out comprehensive gas-dynamical modeling for the emission-line disk within ~70 pc from the nucleus. In comparison with the two previous studies of M84, our analysis includes a more complete treatment of the propagation of emission-line profiles through the telescope and STIS optics, as well as inclusion of the effects of an intrinsic velocity dispersion in the emission-line disk. We find that an intrinsic velocity dispersion is needed in order to match the observed line widths, and we calculate gas-dynamical models both with and without a correction for asymmetric drift. Including the effect of asymmetric drift improves the model fit to the observed velocity field. Our best-fitting model with asymmetric drift gives M BH = (8.5+0.9 -0.8) × 108 M sun (68% confidence). This is a factor of ~2 smaller than the mass often adopted in studies of the M BH-σsstarf and M BH-L relationships. Our result provides a firmer basis for the inclusion of M84 in the correlations between black hole mass and host galaxy properties. Based on observations made with the NASA/ESA Hubble Space Telescope, obtained from the Data Archive at the Space Telescope Science Institute, which is operated by the Association of Universities for Research in Astronomy, Inc., under NASA contract NAS 5-26555. These observations are associated with programs GO-7124 and GO-6094.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2010ApJ...721..762W},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/721/1/762},
  Eprint                   = {1008.0005},
  Keywords                 = {galaxies: active, galaxies: individual: M84 NGC 4347, galaxies: kinematics and dynamics, galaxies: nuclei},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Walsh2015,
  Title                    = {{The Black Hole in the Compact, High-dispersion Galaxy NGC 1271}},
  Author                   = {{Walsh}, J.~L. and {van den Bosch}, R.~C.~E. and {Gebhardt}, K. and {Yildirim}, A. and {G{\"u}ltekin}, K. and {Husemann}, B. and {Richstone}, D.~O.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = aug,
  Pages                    = {183},
  Volume                   = {808},

  Abstract                 = {Located in the Perseus cluster, NGC 1271 is an early-type galaxy with a small effective radius of 2.2 kpc and a large bulge stellar velocity dispersion of 276 km s-1 for its K-band luminosity of 8.9× {10}10 {L}⊙ . We present a mass measurement for the black hole in this compact, high-dispersion galaxy using observations from the Near-infrared Integral Field Spectrometer on the Gemini North telescope assisted by laser guide star adaptive optics, large-scale integral field unit observations with PPAK at the Calar Alto Observatory, and Hubble Space Telescope WFC3 imaging observations. We are able to map out the stellar kinematics both on small spatial scales, within the black hole sphere of influence, and on large scales that extend out to four times the galaxy’s effective radius. We find that the galaxy is rapidly rotating and exhibits a sharp rise in the velocity dispersion. Through the use of orbit-based stellar dynamical models, we determine that the black hole has a mass of ({3.0}-1.1+1.0)× {10}9 {M}⊙ and the H-band stellar mass-to-light ratio is {1.40}-0.11+0.13 {\Upsilon }⊙ (1σ uncertainties). NGC 1271 occupies the sparsely populated upper end of the black hole mass distribution but is very different from the brightest cluster galaxies (BCGs) and giant elliptical galaxies that are expected to host the most massive black holes. Interestingly, the black hole mass is an order of magnitude larger than expectations based on the galaxy’s bulge luminosity but is consistent with the mass predicted using the galaxy’s bulge stellar velocity dispersion. More compact, high-dispersion galaxies need to be studied using high spatial resolution observations to securely determine black hole masses, as there could be systematic differences in the black hole scaling relations between these types of galaxies and the BCGs/giant ellipticals, thereby implying different pathways for black hole and galaxy growth.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...808..183W},
  Archiveprefix            = {arXiv},
  Comment                  = {NIFS},
  Doi                      = {10.1088/0004-637X/808/2/183},
  Eid                      = {183},
  Eprint                   = {1506.05129},
  File                     = {Published version:Walsh2015.pdf:PDF},
  Keywords                 = {black hole physics, galaxies: elliptical and lenticular, cD, galaxies: individual: NGC 1271, galaxies: kinematics and dynamics, galaxies: nuclei, NIFS},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Weijmans2008,
  Title                    = {{The shape of the dark matter halo in the early-type galaxy NGC 2974}},
  Author                   = {{Weijmans}, A.-M. and {Krajnovi{\'c}}, D. and {van de Ven}, G. and {Oosterloo}, T.~A. and {Morganti}, R. and {de Zeeuw}, P.~T.},
  Journal                  = {\mnras},
  Year                     = {2008},

  Month                    = feb,
  Pages                    = {1343-1358},
  Volume                   = {383},

  Abstract                 = {We present HI observations of the elliptical galaxy NGC 2974, obtained with the Very Large Array. These observations reveal that the previously detected HI disc in this galaxy is in fact a ring. By studying the harmonic expansion of the velocity field along the ring, we constrain the elongation of the halo and find that the underlying gravitational potential is consistent with an axisymmetric shape. We construct mass models of NGC 2974 by combining the HI rotation curve with the central kinematics of the ionized gas, obtained with the integral-field spectrograph SAURON. We introduce a new way of correcting the observed velocities of the ionized gas for asymmetric drift, and hereby disentangle the random motions of the gas caused by gravitational interaction from those caused by turbulence. To reproduce the observed flat rotation curve of the HI gas, we need to include a dark halo in our mass models. A pseudo-isothermal sphere provides the best model to fit our data, but we also tested an NFW halo and modified Newtonian dynamics, which fit the data marginally worse. The mass-to-light ratio M/LI increases in NGC 2974 from 4.3Msolar/Lsolar,I at one effective radius to 8.5Msolar/Lsolar,I at 5Re. This increase of M/L already suggests the presence of dark matter: we find that within 5Re at least 55 per cent of the total mass is dark.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008MNRAS.383.1343W},
  Archiveprefix            = {arXiv},
  Comment                  = {Velocity field, isothermal sphere},
  Doi                      = {10.1111/j.1365-2966.2007.12680.x},
  Eprint                   = {0711.1775},
  File                     = {Published version:Weijmans2008.pdf:PDF},
  Keywords                 = {NGC 2974},
  Owner                    = {sinead},
  Timestamp                = {2015.12.14}
}

@Article{Williams2009,
  Title                    = {{Kinematic constraints on the stellar and dark matter content of spiral and S0 galaxies}},
  Author                   = {{Williams}, M.~J. and {Bureau}, M. and {Cappellari}, M.},
  Journal                  = {\mnras},
  Year                     = {2009},

  Month                    = dec,
  Pages                    = {1665-1689},
  Volume                   = {400},

  Abstract                 = {We present mass models of a sample of 14 spiral and 14 S0 galaxies that constrain their stellar and dark matter content. For each galaxy, we derive the stellar mass distribution from near-infrared photometry under the assumptions of axisymmetry and a constant KS-band stellar mass-to-light ratio . To this we add a dark halo assumed to follow a spherically symmetric Navarro, Frenk and White profile and a correlation between concentration and dark mass within the virial radius, MDM. We solve the Jeans equations for the corresponding potential under the assumption of constant anisotropy in the meridional plane, βz. By comparing the predicted second velocity moment to observed long-slit stellar kinematics, we determine the three best-fitting parameters of the model: and βz. These simple axisymmetric Jeans models are able to accurately reproduce the wide range of observed stellar kinematics, which typically extend to ~2-3Re or, equivalently, ~0.5-1R25. Although our sample contains barred galaxies, we argue a posteriori that the assumption of axisymmetry does not significantly bias our results. We find a median stellar mass-to-light ratio at KS-band of with an rms scatter of 0.31. We present preliminary comparisons between this large sample of dynamically determined stellar mass-to-light ratios and the predictions of stellar population models. The stellar population models predict slightly lower mass-to-light ratios than we measure. The mass models contain a median of 15 per cent dark matter by mass within an effective radius Re (defined here as the semimajor axis of the ellipse containing half the KS-band light) and 49 per cent within the optical radius R25. Dark and stellar matter contribute equally to the mass within a sphere of radius 4.1Re or 1.0R25. There is no evidence of any significant difference in the dark matter content of the spirals and S0s in our sample. Models without dark matter are also able to satisfactorily reproduce the observed kinematics in most cases. The improvement when a halo is added is statistically significant, however, and the stellar mass-to-light ratios of mass models with dark haloes match the independent expectations of stellar population models better.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2009MNRAS.400.1665W},
  Archiveprefix            = {arXiv},
  Comment                  = {JAM},
  Doi                      = {10.1111/j.1365-2966.2009.15582.x},
  Eprint                   = {0909.0680},
  Keywords                 = {galaxies: elliptical and lenticular, cD , galaxies: fundamental parameters , galaxies: kinematics and dynamics , galaxies: spiral , galaxies: stellar content , dark matter},
  Owner                    = {sinead},
  Primaryclass             = {astro-ph.GA},
  Timestamp                = {2015.12.18}
}

@Article{Wong2004,
  Title                    = {{A Search for Kinematic Evidence of Radial Gas Flows in Spiral Galaxies}},
  Author                   = {{Wong}, T. and {Blitz}, L. and {Bosma}, A.},
  Journal                  = {\apj},
  Year                     = {2004},

  Month                    = apr,
  Pages                    = {183-204},
  Volume                   = {605},

  Abstract                 = {CO and H I velocity fields of seven nearby spiral galaxies, derived from radio-interferometric observations, are decomposed into Fourier components whose radial variation is used to search for evidence of radial gas flows. Additional information provided by optical or near-infrared isophotes is also considered, including the relationship between the morphological and kinematic position angles. To assist in interpreting the data, we present detailed modeling that demonstrates the effects of bar streaming, inflow, and a warp on the observed Fourier components. We find in all of the galaxies evidence for either elliptical streaming or a warped disk over some range in radius, with deviations from pure circular rotation at the level of ~20-60 km s-1. Evidence for kinematic warps is observed in several cases well inside R25. No unambiguous evidence for radial inflows is seen in any of the seven galaxies, and we are able to place an upper limit of ~5-10 km s-1 (3%-5% of the circular speed) on the magnitude of any radial inflow in the inner regions of NGC 4414, NGC 5033, and NGC 5055. We conclude that the inherent nonaxisymmetry of spiral galaxies is the greatest limitation to the direct detection of radial inflows.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2004ApJ...605..183W},
  Comment                  = {CO/HI map},
  Doi                      = {10.1086/382215},
  Eprint                   = {astro-ph/0401187},
  Keywords                 = {NGC 4414},
  Owner                    = {sinead},
  Timestamp                = {2015.12.15}
}

@Article{Yildirim2016,
  Title                    = {{The massive dark halo of the compact early-type galaxy NGC 1281}},
  Author                   = {{Y{\i}ld{\i}r{\i}m}, A. and {van den Bosch}, R.~C.~E. and {van de Ven}, G. and {Dutton}, A. and {L{\"a}sker}, R. and {Husemann}, B. and {Walsh}, J.~L. and {Gebhardt}, K. and {G{\"u}ltekin}, K. and {Mart{\'{\i}}n-Navarro}, I. },
  Journal                  = {\mnras},
  Year                     = {2016},

  Month                    = feb,
  Pages                    = {538-553},
  Volume                   = {456},

  Abstract                 = {We investigate the compact, early-type galaxy NGC 1281 with integral field unit observations to map the stellar line-of-sight velocity distribution (LOSVD) out to five effective radii and construct orbit-based dynamical models to constrain its dark and luminous matter content. Under the assumption of mass-follows-light, the H-band stellar mass-to-light ratio (M/L) is Υ⋆ = 2.7 ± 0.1 Υ⊙, and higher than expected from our stellar population synthesis fits with either a canonical Kroupa (Υ⋆ = 1.3 Υ⊙) or Salpeter (Υ⋆ = 1.7 Υ⊙) stellar initial mass function. Such models also cannot reproduce the details of the LOSVD. Models with a dark halo recover the kinematics well and indicate that NGC 1281 is dark matter dominated, making up ˜ 90 per cent of the total enclosed mass within the kinematic bounds. Parametrized as a spherical NFW profile, the dark halo mass is 11.5 ≤ log(MDM/M⊙) ≤ 11.8 and the stellar M/L is 0.6 ≤ Υ⋆/Υ⊙ ≤ 1.1. However, this M/L is lower than predicted by its old stellar population. Moreover, the halo mass within the kinematic extent is 10 times larger than expected based on Λ-cold-dark-matter predictions, and an extrapolation yields cluster-sized dark halo masses. Adopting Υ⋆ = 1.7 Υ⊙ yields more moderate dark halo virial masses, but these models fit the kinematics worse. A non-NFW model might solve the discrepancy between the unphysical consequences of the best-fitting dynamical models and models based on more reasonable assumptions for the dark halo and stellar M/L, which are disfavoured according to our parameter estimation.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016MNRAS.456..538Y},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stv2665},
  Eprint                   = {1511.03131},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: haloes, galaxies: kinematics and dynamics, galaxies: structure, dark matter},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@Article{Yildirim2015,
  Title                    = {{MRK 1216 and NGC 1277 - an orbit-based dynamical analysis of compact, high-velocity dispersion galaxies}},
  Author                   = {{Y{\i}ld{\i}r{\i}m}, A. and {van den Bosch}, R.~C.~E. and {van de Ven}, G. and {Husemann}, B. and {Lyubenova}, M. and {Walsh}, J.~L. and {Gebhardt}, K. and {G{\"u}ltekin}, K.},
  Journal                  = {\mnras},
  Year                     = {2015},

  Month                    = sep,
  Pages                    = {1792-1816},
  Volume                   = {452},

  Abstract                 = {We present a dynamical analysis to infer the structural parameters and properties of the two nearby, compact, high-velocity dispersion galaxies MRK 1216 and NGC 1277. Combining deep Hubble Space Telescope imaging, wide-field integral field unit stellar kinematics, and complementary long-slit spectroscopic data out to three effective radii, we construct orbit-based models to constrain their black hole masses, dark matter content and stellar mass-to-light ratios. We obtain a black hole mass of log(M•/M⊙) = 10.1_{-0.2}^{+0.1} for NGC 1277 and an upper limit of log(M•/M⊙) = 10.0 for MRK 1216, within 99.7 per cent (3σ) confidence. The stellar mass-to-light ratios span a range of ΥV = 6.5_{-1.5}^{+1.5} in NGC 1277 and ΥH = 1.8_{-0.8}^{+0.5} in MRK 1216 and are in good agreement with single stellar population models of a single power-law Salpeter initial mass function. Even though our models do not place strong constraints on the dark halo parameters, they suggest that dark matter is a necessary ingredient in MRK 1216, with a dark matter contribution of 22^{+30}_{-20} per cent to the total mass budget within one effective radius. NGC 1277, on the other hand, can be reproduced without the need for a dark halo, and a maximal dark matter fraction of 13 per cent within the same radial extent. In addition, we investigate the orbital structures of both galaxies, which are rotationally supported and consistent with photometric multi-Sérsic decompositions, indicating that these compact objects do not host classical, non-rotating bulges formed during recent (z ≤ 2) dissipative events or through violent relaxation. Finally, both MRK 1216 and NGC 1277 are anisotropic, with a global anisotropy parameter δ of 0.33 and 0.58, respectively. While MRK 1216 follows the trend of fast-rotating, oblate galaxies with a flattened velocity dispersion tensor in the meridional plane of the order of βz ˜ δ, NGC 1277 is highly tangentially anisotropic and seems to belong kinematically to a distinct class of objects.},
  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015MNRAS.452.1792Y},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stv1381},
  Eprint                   = {1506.06762},
  Keywords                 = {galaxies: elliptical and lenticular, cD, galaxies: kinematics and dynamics, galaxies: structure, dark matter},
  Owner                    = {sinead},
  Timestamp                = {2015.12.21}
}

@comment{jabref-meta: fileDirectory:/home/sinead/Desktop/JabRef/Papers
;}

@comment{jabref-meta: groupsversion:3;}

@comment{jabref-meta: groupstree:
0 AllEntriesGroup:;
1 ExplicitGroup:My galaxies\;0\;;
2 ExplicitGroup:NGC 4414\;0\;Fisher2009\;Gurovich2010\;Heald2011\;Saty
apal2008\;Vallejo2002\;Wong2004\;deBlok2014\;;
1 ExplicitGroup:SMBHs - Dynamics\;0\;Brok2015\;Cappellari2002a\;Cretto
n1999\;Drehmer2015\;Gebhardt2011\;Gueltekin2009a\;Krajnovic2009a\;Lyub
enova2008\;Nowak2008\;Rusli2013\;Seth2014\;Walsh2010\;Walsh2015\;Yildi
rim2015\;Yildirim2016\;vandenBosch2010\;;
1 ExplicitGroup:Coevolution\;0\;2016arXiv160102613G\;Antonini2015\;Fer
re-Mateu2015\;Fontanot2015\;Gueltekin2009\;Kormendy2013\;Reines2015\;S
chulze2011\;;
1 ExplicitGroup:Pseudobulges\;0\;Fisher2009\;;
1 ExplicitGroup:SMBH - Others\;0\;Kuo2011\;Oka2016\;;
1 ExplicitGroup:PotW\;0\;Antonini2015\;Husemann2016\;;
1 ExplicitGroup:SINFONI\;0\;;
1 ExplicitGroup:BH evolution\;0\;;
1 ExplicitGroup:Methods\;0\;Cappellari2002\;Cappellari2002b\;Cappellar
i2003\;Cappellari2004\;Cappellari2008\;Carollo1997a\;Falcon-Barroso201
1\;Freudling2013\;Jeans1922\;McDermid2006\;McDermid2006a\;McDermid2015
\;Qian1995\;Sanchez-Blazquez2006\;Scott2013\;Shetty2015\;Weijmans2008\
;vandenBosch2010\;;
1 ExplicitGroup:Galaxy Dynamics\;0\;Cappellari2009\;;
1 ExplicitGroup:DM\;0\;Rusli2013\;Williams2009\;Yildirim2016\;;
1 ExplicitGroup:Review\;0\;Cappellari2016\;Cole2016\;Kormendy2013\;;
1 ExplicitGroup:Interesting\;0\;Do2014\;;
}


